A Mechanism for Producing Aligned Latent Spaces with Autoencoders

Aligned latent spaces, where meaningful semantic shifts in the input space correspond to a translation in the embedding space, play an important role in the success of downstream tasks such as unsupervised clustering and data imputation. In this work, we prove that linear and nonlinear autoencoders produce aligned latent spaces by stretching along the left singular vectors of the data. We fully characterize the amount of stretching in linear autoencoders and provide an initialization scheme to arbitrarily stretch along the top directions using these networks. We also quantify the amount of stretching in nonlinear autoencoders in a simplified setting. We use our theoretical results to align drug signatures across cell types in gene expression space and semantic shifts in word embedding spaces.

==> Alignment via Over-parameterized Autoencoders/checklist.tex <==



\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Sections \ref{sec: Stretching} and \ref{sec: Autoencoders}.}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{sec: Conclusion}} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section \ref{sec: Conclusion}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{All assumptions are stated in Sections \ref{sec: Stretching} and  \ref{sec: Autoencoders}} 
	\item Did you include complete proofs of all theoretical results?
    \answerYes{All proofs are provided in the Appendix.} 
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} \textcolor{red}{TODO link to code}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} 
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}. 
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We provide this in the Appendix.} 
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{All citations for datasets are present in \ref{sec: Applications}.}
  \item Did you mention the license of the assets?
    \answerYes{See citations discussed above.} 
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We provide a link to our code in \textcolor{red}{TODO}.} 
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{} 
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> Alignment via Over-parameterized Autoencoders/sections/abstract.tex <==
Aligned latent spaces, where meaningful semantic shifts in the input space correspond to a translation in the embedding space, play an important role in the success of downstream tasks such as unsupervised clustering and data imputation.  In this work, we prove that linear and nonlinear autoencoders produce aligned latent spaces by stretching along the left singular vectors of the data.  We fully characterize the amount of stretching in linear autoencoders and provide an initialization scheme to arbitrarily stretch along the top directions using these networks.  We also quantify the amount of stretching in nonlinear autoencoders in a simplified setting.  We use our theoretical results to align drug signatures across cell types in gene expression space and semantic shifts in word embedding spaces.\footnote{Code available at \small{\url{https://github.com/uhlerlab/latent_space_alignment}}.}
% \footnote{Code available at \small{\url{https://github.com/alignedlatentspaces/latent_space_alignment}}.}


==> Alignment via Over-parameterized Autoencoders/sections/acks.tex <==
This work was partially supported by NSF (DMS-1651995), ONR (N00014-17-1-2147 and N00014-18-1-2765), the MIT-IBM Watson AI Lab, and a Simons Investigator Award to C. Uhler. The Titan Xp used for this research was donated by the NVIDIA Corporation.   

==> Alignment via Over-parameterized Autoencoders/sections/alignment_section/alignment.tex <==
In this section, we prove that over-parameterized, 1-hidden layer linear autoencoders trained using gradient flow from an asymmetric spectral initialization produce embeddings that are stretched along the top left singular vectors of the data.  We then prove that a similar phenomenon occurs for non-linear 1-hidden layer ReLU autoencoders trained on two data points.  We lastly connect this stretching to alignment of directions of interest in the latent space by demonstrating that asymmetrically initialized autoencoders align the major axes of a Gaussians in the mixture model from Section \ref{sec: Stretching}.  We begin with a review of autoencoder preliminaries. 

\subsection{Autoencoder Preliminaries}
\input{sections/preliminaries}

\subsection{Stretching in Over-parameterized Linear Autoencoders}
\input{sections/alignment_section/gradient_flow}

\subsection{Stretching in Over-parameterized Nonlinear ReLU Autoencoders}
\input{sections/alignment_section/non_linear}

==> Alignment via Over-parameterized Autoencoders/sections/alignment_section/gradient_flow.tex <==
We begin by deriving the gradient flow solution for 1-hidden layer autoencoders from arbitrary spectral initialization \cite{ImplictRegularizationBach, Saxe2014, Saxe2019}.  By exploring how initialization impacts the singular values of the gradient flow solution, we  derive a simple, computationally tractable asymmetric spectral initialization scheme that yields stretching along the top left singular vectors of the training data. 

\begin{theorem}
\label{theorem: two layer linear autoencoder}
Let $f(x) = ABx$ denote a neural network with $A, B \in \mathbb{R}^{d \times d}$ and $x \in \mathbb{R}^{d}$, and let $X \in \mathbb{R}^{d \times n}$ denote the training data.  If $A, B$ are initialized according to the spectral initialization (Definition \ref{def: Spectral Initialization}), then gradient flow on $A, B$ converges to: 
\begin{align*}
    A^{(\infty)} &= U_X \Sigma_A^{(\infty)} U_X^T ~~;~~ B^{(\infty)} = U_X \Sigma_B^{(\infty)} U_X^T,  ~~  \\
    {\Sigma_{B}}_{i,i}^{(\infty)} &= \sqrt{\frac{({\Sigma_B^{(0)}}_{i,i}^2 - {\Sigma_A^{(0)}}_{i,i}^2)}{2} + \sqrt{1 + \frac{({\Sigma_B^{(0)}}_{i,i}^2 - {\Sigma_A^{(0)}}_{i,i}^2)^2}{4}}} ~~ ; ~~ {\Sigma_{A}^{(0)}}_{i,i}^{(\infty)} = {\Sigma_{B}^{(0)}}_{i,i}^{-1}.
\end{align*}
\end{theorem}

The full proof is provided in Appendix \ref{appendix: Gradient flow solution linear autoencoders}; it is inspired by the proof strategy used in \cite{RadhakrishnanOPAMemory}.  We now provide an initialization scheme that leads to alignment in the latent space.   

% As discussed in \ref{sec: Preliminaries}, when $\Sigma_A^{(0)} =  \Sigma_B^{(0)}$, the result recovers the fact that linear autoencoders project onto the subspace spanned by the data.  In particular, if $X$ has full rank, $\Sigma_B = I$ at the end of training and hence does not generate aligned embeddings in the latent space.  


\noindent \textbf{Asymmetric Spectral Initialization.} In order to generate aligned embeddings, we now turn to the following asymmetric spectral initialization.  Provided that $B^{(0)}$ is a polynomial in $\frac{1}{n}XX^T + I$ and $A^{(0)} = \mathbf{0}$, Theorem \ref{theorem: two layer linear autoencoder} guarantees that $B$ stretches inputs along the top directions given by the top left singular vectors of the training data, $X$.  This is formalized in the following corollary.

\begin{corollary}
\label{corollary: Polynomial Stretching} 
Let $f(x) = ABx$ denote a neural network with $A, B \in \mathbb{R}^{d \times d}$ and $x \in \mathbb{R}^{d}$, and let $U_X \Sigma_X V_X^T$ denote the SVD of $X$. Let $A^{(0)} = \mathbf{0}$ and $B^{(0)}$  be a polynomial in $\frac{1}{n}XX^T + I$.  Let $\sigma_i(B^{(t)})$ denote the $i$\textsuperscript{th} singular value of $B^{(t)}$.  Then $B^{(\infty)}$ given by gradient flow satisfies: 
% \begin{align*}
%     & A^{(\infty)} = U_X \Sigma_A^{(\infty)} U_X^T ~~;~~ B^{(\infty)} = U_X \Sigma_B^{(\infty)} U_X^T  ~~ \text{with} ~~ {\Sigma_{B}}_{i,i}^{(\infty)}   \geq \sigma_i(B^{(0)}) \geq 1
% \end{align*}
\begin{align*}
   \sigma_i(B^{(\infty)}) \geq \sigma_i(B^{(0)}) \geq 1.
\end{align*}
\end{corollary}

\textbf{Remarks.}  
 From Corollary \ref{corollary: Polynomial Stretching}, we find that $B^{(\infty)}$ after gradient descent from an asymmetric spectral initialization will stretch along the top singular vectors even more than $B^{(0)}$. We note that this property does not necessarily hold for symmetric spectral initialization.  Moreover, we can achieve an arbitrary amount of stretching along the top singular vectors of the data by scaling the degree of the matrix polynomial used to initialize $B^{(0)}$.  Finally, unlike general spectral initialization, our asymmetric initialization above does not require computing any singular vectors, and hence is readily usable in practice.

% Moreover, Corollary \ref{corollary: Polynomial Stretching} implies that linear autoencoders only increase the amount of stretching given by the initialization \textcolor{red}{sentence unclear}.  

\subsection{Aligning Latent Spaces with Linear Autoencoders}
Returning to the example of a Gaussian mixture from Section \ref{sec: Stretching}, we now use Theorem \ref{theorem: two layer linear autoencoder} to prove that asymmetrically initialized linear autoencoders can promote alignment. Specifically, we revisit the setting of Corollary \ref{corollary: two gaussians}, which consisted of two Gaussians whose major axes are nearly orthogonal. By generating $B$ from our linear autoencoder, we find that autoencoding will align the major axes of these Gaussians (Proof in Appendix \ref{appendix: two gaussians after autoencoding}).
\begin{corollary}
\label{corollary: two gaussians after autoencoding}
In the setting of Corollary \ref{corollary: two gaussians}, set $B$ to be the encoding matrix of an autoencoder $f(x)=ABx$ after gradient flow where $A$ is initialized to $0$ and $B$ is initialized to $(\frac{1}{n}XX^T)^k$. Then, as n tends to infinity,
$$\cos(Bq_{\Sigma_1}, Bq_{\Sigma_2}) = \frac{2 + \gamma \sqrt{c^2 + 4}}{2\gamma + \sqrt{c^2 + 4}} , \quad \gamma = \frac{(\alpha^2 - \beta^2)}{(\alpha^2 + \beta^2)},$$
where
$$\alpha = \lambda_1(B) = \sqrt{\frac{(c+7)^{2k}}{2} + \sqrt{1 + \frac{(c+7)^{4k}}{4}}}, \;\beta = \lambda_2(B) = \sqrt{\frac{(c+3)^{2k}}{2} + \sqrt{1 + \frac{(c+3)^{4k}}{4}}}.$$
Thus the alignment of $q_1$ and $q_2$ will increase, and this alignment can be arbitrarily boosted by encoding with higher degree $k$.
\end{corollary}

Since autoencoders with asymmetrical spectral initialization stretch along the top directions of the dataset, we can use them to boost  alignment while allowing for perfect reconstruction via decoding. In Section \ref{sec: Applications}, we explore how linear autoencoders can be used to align real-world datasets. 

% The question remains as to how this stretching is connected to the alignment phenomenon in the latent space.  The following example demonstrates that power iteration (i.e. choosing a large enough polynomial in $XX^T + I$) can boost the  alignment of vectors.

% \begin{figure}
%     \centering
%     \includegraphics[width=1\textwidth]{Figures/ToyDataAlignment.pdf}
%     \caption{Boosting alignment in the latent space for a synthetic dataset consisting of 4 circles of 100 points each.  We measure alignment by first computing the difference between points in intersecting circles (shown as black vectors) and then computing the cosine similarity between these difference vectors. (a) A visualization of the original dataset. (b) A visualization of the latent space after training a two layer linear autoencoder $f(x) = A B x$ from initialization $A^{(0)} = 0$ and $B^{(0)} = \left( \frac{1}{n} XX^T + I \right)^{10}$. While the cosine similarity in the original space is .1, the cosine similarity in the latent space is .9.}
%     \label{fig:toy data alignment}
% \end{figure}


==> Alignment via Over-parameterized Autoencoders/sections/alignment_section/non_linear.tex <==
In the previous section, we proved that asymmetrically initialized linear over-parameterized autoencoders stretch along the top left singular vectors of the data.  We now provide a proof that the same is true for asymmetrically initialized over-parameterized ReLU autoencoders in a simplified setting with two opposing datapoints. 
We use gradient flow to compute the closed forms of  $A^{(\infty)}, B^{(\infty)}$. Since the dataset $[-x, x]$ has exactly one singular vector with non-zero singular value (i.e $x$), we compute the stretching factor as the magnitude of the new embedding of $x$ (i.e $||Bx||_2$).

\begin{theorem}
Let $f(x) = A\phi(Bx)$ be a neural network with $A \in \mathbb{R}^{d \times 2d}, B \in \mathbb{R}^{2d \times d}$, and $\phi$ as a ReLU activation. For some $x \in \mathbb{R}^{d}$ with $\eta = ||x||_2^2$, let $X = \{x, -x\}$ denote the training set. 
Let $A$ and $B$ be initialized as
$$A^{(0)} = 0, \;B^{(0)} = \begin{bmatrix} xx^T \\ -xx^T\end{bmatrix}.$$
Then after using gradient flow, we have that $A^{(\infty)} = \alpha  (B^{(0)})^T$ and  $B^{(\infty)} = \beta B^{(0)}$, where
$$\beta^2 = \frac{1}{2} \left(\frac{\sqrt{\eta^4 + 4}}{\eta^2} +1\right), \;\alpha \beta = \frac{1}{\eta}.$$
Moreover, gradient flow will stretch the embedding of $x$ by a quadratic factor of $\eta$:
$$ ||Bx||_2^2 = \eta^2 \left(\frac{\sqrt{\eta^4 + 4}}{\eta^2} +1\right) \|x\|^2.$$
\label{theorem:non_linear}
\end{theorem}
The full proof can be found in Appendix \ref{appendix: non_linear}, but proceeds through gradient flow analysis similar to Theorem \ref{theorem: two layer linear autoencoder}. As in the linear setting, we find that by asymmetrically initializing $A$ and $B$, we can stretch the embedding of the dataset along the top left singular vector.  

==> Alignment via Over-parameterized Autoencoders/sections/alignment_section/two_gaussians_after_autoencoding.tex <==
% \begin{corollary}
% In the setting of Corollary \ref{corollary: two gaussians}, set $B$ to be the encoding matrix of an autoencoder $f(x)=ABx$ after gradient descent where $A$ is initialized to $0$ and $B$ is initialized to $(\frac{1}{n}XX^T)^k$. Then, as n tends to infinity, the cosine similarity of $q_1$ and $q_2$ (the major axes of the individual gaussians) after embedding with $B$ is converges almost surely to 
% $$\cos \theta' = \frac{(B q_{\Sigma_1})^T B q_{\Sigma_1}}{||B q_{\Sigma_1}||_2 ||B q_{\Sigma_1}||_2} = \frac{2 + \gamma \sqrt{c^2 + 4}}{2\gamma + \sqrt{c^2 + 4}} , \quad \gamma = \frac{(\alpha^2 - \beta^2)}{(\alpha^2 + \beta^2)}$$
% where
% $$\alpha = \lambda_1(B) = \sqrt{\frac{(c+7)^{2k}}{2} + \sqrt{1 + \frac{(c+7)^{4k}}{4}}}, \beta = \lambda_2(B) = \sqrt{\frac{(c+3)^{2k}}{2} + \sqrt{1 + \frac{(c+3)^{4k}}{4}}}$$
% Thus the alignment of $q_1$ and $q_2$ will increase, and this alignment can be arbitrarily boosted by encoding with higher degree $k$.
% \end{corollary}


\begin{proof}
Let $\lambda_i$ be the $i$th eigenvalue of $XX^T$. By Theorem \ref{theorem: two layer linear autoencoder}, if we initialize $A^{(0)}=0$ and  $B^{(0)} = (\frac{1}{n} XX^T) = U_X \Sigma_B U_X^T$, then after gradient descent we have:
$$B = U_X \Sigma_B U_X^T, (\Sigma_B)_i = \sqrt{\frac{\lambda_i^{2}}{2} + \sqrt{1 + \frac{\lambda_i^{4}}{4}}}.$$

For our particular setting, from Corollary \ref{appendis: two gaussians with xxt}, we know that $B^{(0)}$ converges as $n$ tends towards infinity:
$$B^{(0)} \xrightarrow{a.s} I + 2 J = (c + 3) I + 4\hat{v}\hat{v}^T$$
with eigenvectors $\hat{v} = \frac{[1,1]^T}{\sqrt{2}}$ and $\hat{u} = [1, -1]^T/\sqrt{2}$ with eigenvalues:
$\lambda_1 = (c + 7), \lambda_2 = (c+3)$. 

Moreover, we note that the mapping from $B^{(0)} \rightarrow B$ is continuous since it is a composition of applying the matrix square root and matrix polynomials, which are both continuous. Then using the continuous mapping theorem, we have that $B$ converges almost surely to $\bar{B}$, where $\bar{B}$ can be expressed as 
$$U_X = \begin{bmatrix} \hat{v} & \hat{u} \end{bmatrix} = \frac{1}{\sqrt{2}}\begin{bmatrix}1 & 1 \\ 1 & -1\end{bmatrix}, \quad \Sigma_{\bar{B}} =\begin{bmatrix} \alpha &  0 \\ 0 & \beta \end{bmatrix}, \quad \bar{B} = U_X \Sigma_{\bar{B}} U_X^T$$
for
$$\alpha = (\Sigma_{\bar{B}})_1 = \sqrt{\frac{(c+7)^{2}}{2} + \sqrt{1 + \frac{(c+7)^{4}}{4}}}, \beta = (\Sigma_{\bar{B}})_2 = \sqrt{\frac{(c+3)^{2}}{2} + \sqrt{1 + \frac{(c+3)^{4}}{4}}}.$$

We thus have that that:
$$\cos(Bq_{\Sigma_1}, Bq_{\Sigma_2})  \xrightarrow{a.s} \cos(\bar{B}q_{\Sigma_1}, \bar{B}q_{\Sigma_2})  = \frac{2 + \gamma \sqrt{c^2 + 4}}{2\gamma + \sqrt{c^2 + 4}} , \quad \gamma = \frac{(\alpha^2 - \beta^2)}{(\alpha^2 + \beta^2)}$$
for the above $\alpha$ and $\beta$. Moreover, as $k$ increases, the $\gamma$ goes up, and  $Bq_{\Sigma_1}$ and $Bq_{\Sigma_2}$ become more aligned. 
\end{proof}

==> Alignment via Over-parameterized Autoencoders/sections/applications_section/applications.tex <==
Thus far, we have demonstrated that autoencoders can align directions of interest in the latent space by stretching along the left singular vectors of the data.  While we primarily focused on proving this for the case of a Gaussian mixture model, we now apply our theoretical results to produce autoencoders that align semantic/syntactic directions in word embedding space and drug signatures in gene expression space.  

\subsection{Alignment of GloVe Embeddings}
\input{sections/applications_section/glove}

\subsection{Drug Signature Alignment in CMap}
\input{sections/applications_section/cmap}


==> Alignment via Over-parameterized Autoencoders/sections/applications_section/cmap.tex <==

Finally, we apply our theoretical results to gene expression data from CMap \cite{CMap} to boost the alignment of drug signatures, i.e the difference in gene expression for a cell type at control and after applying the drug. Prior work \cite{COVIDAutoencoding} demonstrated that 1-hidden layer over-parameterized autoencoders with Leaky ReLU \cite{LeakyReLU} activation produced pre-activation latent spaces which aligned drug signatures across cell types.  The boost in alignment was evaluated by plotting the cosine similarity of drug signatures across cell types in the original and the autoencoded latent space.  

Following the setting of \cite{COVIDAutoencoding}, we measure the alignment of drug signatures between MCF7 and A549 cell types using linear and nonlinear autoencoders (Figure \ref{fig: Drug Signature Alignment}). We find that linear autoencoders with asymmetric spectral initialization can boost alignment even beyond the alignment given by the Leaky ReLU autoencoder in \cite{COVIDAutoencoding}. Moreover, using a high degree polynomial for asymmetric initialization (i.e., degree 30 in Figure~\ref{fig: Drug Signature Alignment}c) leads to all drug signatures being nearly perfectly aligned.  

% Finally, we apply our theoretical results to boost the alignment of drug signatures across cell types from CMap \cite{CMap}.  Prior work \cite{COVIDAutoencoding} demonstrated that 1-hidden layer over-parameterized autoencoders with Leaky ReLU \cite{LeakyReLU} activation produced pre-activation latent spaces in which the drug signatures, i.e. the difference in gene expression between the cell type after drug and cell type at control, were aligned across cell types.  The increase alignment was demonstrated by plotting the difference between cosine similarity between drug signatures across cell types in the original vs. latent space.  In Figure \ref{fig: Drug Signature Alignment}a, we  reproduce the plot of \cite{COVIDAutoencoding} for drug signatures between MCF7 and A549 cell types and verify the boost in alignment.  

% In Figures \ref{fig: Drug Signature Alignment}b and c, in accordance with our preceding theory, we demonstrate that using  linear autoencoders with asymmetric spectral initialization again leads to an increase in alignment on the same task.  Moreover, using a high degree polynomial for asymmetric initialization (i.e. degree 30 in Figure \ref{fig: Drug Signature Alignment}c) leads to all drug signatures having cosine similarity near $-1$ or $1$.  


\begin{figure}
    \captionsetup[subfigure]{justification=centering}   
    \centering
    \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\textwidth]{Figures/DrugLeakyReLU.pdf}
    \centering
    \caption{Leaky ReLU Autoencoder}
    \end{subfigure}
    \begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/DrugLinearDeg10.pdf}
    \caption{Linear Autoencoder (k=10)}
    \end{subfigure}
    \begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/DrugLinearDeg30.pdf}
    \caption{Linear Autoencoder (k=30)}
    \end{subfigure}
    \caption{Alignment of drug signatures across 2 cell types (MCF7 and A549) using (a) LeakyReLU autoencoders from \cite{COVIDAutoencoding} and (b,c) linear autoencoders with asymmetric spectral initialization. Using linear autoencoders can lead to greater alignment than using a LeakyReLU autoencoder.}
    \label{fig: Drug Signature Alignment}
\end{figure}



% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/DrugSimilarity.pdf}
%     \caption{Alignment of drug signatures across 2 cell types (MCF7 and A549 cell types) using (a) LeakyReLU autoencoders from \cite{COVIDAutoencoding} and (b,c) linear autoencoders with asymmetric spectral initialization. Using linear autoencoders can lead to greater alignment than using a LeakyReLU autoencoder.
%     % Linear autoencoders with asymmetric spectral initialization produce latent spaces in which drug signatures are aligned across 2 cell types (MCF7 and A549 cell types).  (a) Leaky ReLU Autoencoders from \cite{COVIDAutoencoding} align drug signatures across cell types. (b, c) We show that linear autoencoders with asymmetric initialization lead to a greater boost in alignment of drug signatures cell types than nonlinear autoencoders.
%     }
%     \label{fig: Drug Signature Alignment}
% \end{figure}

==> Alignment via Over-parameterized Autoencoders/sections/applications_section/glove.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\textwidth]{Figures/original_negation.pdf}
     \caption{Original Space}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\textwidth]{Figures/negation_linear_ae_2.pdf}
     \caption{Linear Autoencoder (k=2)}
    \end{subfigure}
    \caption{We visualize the embeddings of several pairs of words with a negation relationship using MDS both in the original space and linearly autoencoded space (k=2). The linearly autoencoded space aligns the word pairs to point in the same direction.}
    \label{fig:negation_alignment}
    % \vspace{-1.5em}
\end{figure}


In this section, we apply our theory to align semantic/syntactic directions in GloVe word embeddings \cite{pennington2014glove}. We use 300 dimensional GloVe vectors that were trained on Common Crawl with 840 billion tokens. We consider the embeddings of the 500,000 most frequent words, and encode these embeddings with linear and non-linear autoencoders. Details about our experimental setup and training procedures can be found in Appendix \ref{appendix: experimental_setup}.


\subsubsection{Alignment of Meaningful Directions}
We first consider how autoencoders can align meaningful directions in the GloVe embedding data. We consider word relationships from the Google analogy dataset \cite{mikolov2013linguistic}, which consists of 19,544 question pairs over 14 types of relationships. Such relationships include semantic directions (such as man $\rightarrow$ woman) and syntactic directions (such as cat $\rightarrow$ cats). 

We study how stretching the top singular vectors of the data through autoencoders can align these directions. Prior work suggests that the top singular vectors of GloVe data are closely related to the frequency of a word \cite{mu2017all}. We confirm this finding by plotting, for word embedding $a$, the frequency ranking of that word against its cosine similarity with the singular vector $u_1$ (Appendix \ref{appendix:glove_frequency}). Recall from Lemma \ref{lemma: Alignment Intuition} that, to boost alignment, we would like the the stretching axis to be roughly equally aligned with the directions of interest. Since we consider relationships between words which are independent of word frequency, we suspect that stretching along the top singular vectors of the GloVe will allow us to align word relationships in the data. 

To evaluate alignment in these directions, we randomly draw two word pairs $(a_1, b_1)$ and $(a_2, b_2)$ which capture the same relationship.  We then plot the cosine distances of $b_1 - a_1$ and $b_2 - a_2$ before and after autoencoding (Appendix \ref{appendix: glove_alignment}). We find that autoencoding with either a linear or nonlinear autoencoder boosts alignment of these semantic directions in the latent space.

We can further visualize this alignment by visualizing the latent space before and after autoencoding with multidimensional scaling (MDS). In Figure \ref{fig:negation_alignment}, we visualize the alignment of a subset of the pairs in the relationship ``negation" (e.g aware $\rightarrow$ unaware). We find that autoencoding with both linear and non-linear autoencoders is able to align the direction of negation. We depict the full MDS visualization for negation and demonstrate alignment of other relationships in Appendix \ref{appendix:glove_mds}.


% \textcolor{red}{bold top results?}
\renewcommand{\arraystretch}{0.8}
\begin{table}[t]
    \centering
    \caption{Analogy and word similarity metrics for GloVe data before and after autoencoding. Autoencoding can improve analogy scores without causing a significant degradation in word similarity. }
    \begin{tabular}{l|cc|cc}
    \toprule
        Model & \begin{tabular}{c}\texttt{wsim}\\(MTurk-771)\end{tabular} & \begin{tabular}{c}\texttt{wsim}\\(MEN)\end{tabular}& \begin{tabular}{c}\texttt{analogy}\\(Google)\end{tabular} & \begin{tabular}{c}\texttt{analogy-accuracy}\\(Google)\end{tabular}  \\\midrule
        Original  &   \textbf{0.629} &  \textbf{0.739} & 0.417 & 0.338\\
        Linear AE (k=1) &  0.628 & 0.738 & 0.512 &\textbf{0.382}\\
        Linear AE (k=2) & 0.611 & 0.729 & \textbf{0.656} & 0.322 \\
        Leaky ReLU AE & 0.592 &  0.698 &  0.509 & 0.370\\
        \bottomrule
    \end{tabular}
    \label{tab:glove_metrics}
    % \vspace{-1em}
\end{table}

\subsubsection{Word Analogy Metrics}
To evaluate alignment on a more quantitative level, we study the effect of autoencoding on word analogy tasks. We consider a list of 4-tuples of the form $(a_1, b_1, a_2, b_2)$ which have the analogy relationship $a_1$:$b_1$::$a_2$:$b_2$. One such example might be the embeddings of (men, women, king, queen). 

We evaluate two metrics for word analogy alignment. In the first, \texttt{analogy}, we simply calculate the average cosine similarity $\cos(a_2-a_1, b_2-b_1)$. In the second, \texttt{analogy-accuracy}, we evaluate whether $b_2 = \text{argmax}_{b^*} \cos(b^*, a_2 - a_1 + b_1)$ following \cite{levy2014linguistic}. We form the 4-tuples by combining every possible pair within each relationship in the Google Analogy dataset \cite{mikolov2013linguistic}. 

% \textcolor{red}{Table 1 or Table 2??}
In Table \ref{tab:glove_metrics}, we find that autoencoding substantially boosts the  \texttt{analogy} metric, as semantic directions become more aligned. Intriguingly, we can boost alignment beyond a nonlinear autoencoder by simply using a linear autoencoder with a higher degree $k$. Moreover, we find that encoding the GloVe dataset with a smaller degree linear autoencoder also boosts accuracy on the analogy task. 



\subsection{Word Similarities}
In the previous subsections, we showed that autoencoding word embeddings can align meaningful linguistic directions. Word locality is another important property of word embedding spaces:  similar words should have similar representations. In this section, we show that aligning the space through autoencoding does not significantly degrade the locality of words in the latent space. 

Word similarity datasets are comprised of word pairs along with human annotated ratings of the words' relatedness. We compute the similarity of two words as the cosine similarity between the words' embeddings. Following \cite{chung2017learning}, we evaluate the metric \texttt{wsim} as the Spearman's rank correlation between the rankings computed via cosine similarity and the rankings from the human annotation. 
We use two word-similarity datasets:  Mturk-771 \cite{halawi2012large}, which rates 771 word pairs on a scale of 0 to 5, and MEN \cite{bruni2014multimodal}, which rates 3000 word pairs on a scale of 0 to 50. 

\paragraph*{Reference Point Correction} Word similarity metrics typically compute the cosine similarity of individual embeddings with respect to the origin $o = \mathbf{0}$. However, since autoencoding stretches along the top singular vector, this origin is a poor reference point since it does not stretch along with the rest of the dataset. Instead, we choose a reference point that will also stretch alongside the top principal component: for the original GloVe dataset $X$, we set the reference point to be $o = \lambda_1 u_1$, where $\lambda_1, u_1$ are the top left singular value and vector of $X$. Further considerations on this correction can be found in Appendix \ref{appendix: reference_point_correction}. 

In Table \ref{tab:glove_metrics}, we find that the word similarity metrics remain largely stable after autoencoding, indicating that alignment does not significantly warp the latent space. Thus, autoencoding can align GloVe data without losing important properties such as word locality.  



==> Alignment via Over-parameterized Autoencoders/sections/checklist.tex <==


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Sections \ref{sec: Stretching} and \ref{sec: Autoencoders}.}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{sec: Conclusion}} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section \ref{sec: Conclusion}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{All assumptions are stated in Sections \ref{sec: Stretching} and  \ref{sec: Autoencoders}} 
	\item Did you include complete proofs of all theoretical results?
    \answerYes{All proofs are provided in the Appendix.} 
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We provide a link to our code in the footnote at the end of the Abstract.} 
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} 
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}. 
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We provide this in the Appendix.} 
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{All citations for datasets are present in Section \ref{sec: Applications}.}
  \item Did you mention the license of the assets?
    \answerYes{See citations discussed above.} 
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We provide a link to our code in the footnote at the end of the Abstract.} 
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{} 
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> Alignment via Over-parameterized Autoencoders/sections/discussion.tex <==
In this work, we analyzed a mechanism through which autoencoders with asymmetric spectral initialization  produce aligned latent spaces by stretching along the top singular vectors of the dataset. After fully characterizing the degree of stretching in linear autoencoders, we showed that we can arbitrarily stretch along the top directions by adjusting the initialization.  We further replicated this behavior for nonlinear autoencoders in a simplified setting. We lastly applied our theoretical results to develop autoencoders that align linguistic shifts in word embedding spaces and drug signatures in gene expression data.  

 While we analyzed autoencoders initialized using asymmetric spectral initialization, \cite{COVIDAutoencoding} observed that even the default initialization scheme from PyTorch \cite{PyTorch} can empirically lead to alignment.  An interesting direction of future work would be to provide theoretical guarantees around what initialization regimes in linear and non-linear settings guarantee alignment of semantically meaningful directions after gradient descent. Another interesting avenue would be to characterize alignment of autoencoders in infinite width settings to facilitate analysis of more complex autoencoders. While neural tangent  kernel (NTK) analyses are not readily applicable for understanding latent space analysis, other parameterizations that admit feature learning (such as the $\mu P$ parameterization \cite{GregYangFeatureLearning}) may be more helpful for understanding alignment.

% \textbf{Societal Impact.}  In this work, we presented a theoretical analysis characterizing when and how autoencoders produce aligned latent spaces.  Such theoretical analyses are essential to improving the transparency of models used in practice.  In particular, producing latent spaces in which meaningful semantic shifts are aligned leads to greater intepretability of data representations produced by autoencoders.  Naturally, it is also important to understand which data directions are being aligned and to ensure that directions corresponding to biases inherent in the data are not being reinforced through alignment.  


==> Alignment via Over-parameterized Autoencoders/sections/introduction.tex <==
Modern deep networks are capable of learning rich latent spaces, i.e., vector spaces that capture similarity between data points (Ch.~15 of \cite{goodfellow2016deep}). These learned structured latent spaces play an important role in the success of several downstream inference tasks such as unsupervised clustering \cite{mukherjee2019clustergan}, topic modeling \cite{dieng2020topic}, and classification in low-data regimes \cite{rudolph2019structuring}.  

% For example, representations that capture semantic similarity between data points can be readily applied in downstream tasks such unsupervised clustering \cite{mukherjee2019clustergan} and topic modeling \cite{dieng2020topic}.  Additionally, structured latent spaces in computer vision can improve classification in low-data regimes \cite{rudolph2019structuring}, facilitate anomaly detection \cite{norlander2019latent}, and improve uncertainty calibration for supervised tasks \cite{lee2018simple}.  

For many downstream learning tasks such as those in Figure \ref{fig: Overview Schematic}, a structured latent space in which meaningful semantic directions are \textit{aligned} is particularly useful.  For example, alignment of semantic directions (as in Figure \ref{fig: Overview Schematic}a) can be useful for identifying word analogies or performing word arithmetic with commonly used word embeddings such as GloVE \cite{pennington2014glove} and word2vec \cite{rong2014word2vec}.  

Recent work \cite{COVIDAutoencoding, TheisAutoencoding} empirically demonstrated that autoencoders are capable of automatically producing aligned spaces when embedding gene expression data, but the mechanism through which neural networks produce aligned latent spaces has been unclear.  

\begin{figure}
    \centering
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=.7\textwidth]{Figures/WordSchematic.pdf}
    \caption{Word Embedding Space}
    \end{subfigure}
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=.935\textwidth]{Figures/DrugSchematic.pdf}
    \caption{Gene Expression Embedding Space}
    \end{subfigure}
    %     \begin{subfigure}{0.32\textwidth}
    % \centering
    % \includegraphics[width=\textwidth]{Figures/s3_unaligned.pdf}
    % \caption{Encoding decreases alignment }
    % \end{subfigure}
    \caption{Examples of aligned latent spaces. (a) Alignment of semantic directions (i.e. negation) in word embeddings. (b) Alignment of drug signatures across cell types in gene expression embeddings.}
    \label{fig: Overview Schematic}
\end{figure}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9\textwidth]{Figures/OverviewSchematic.pdf} 
%     % \includegraphics[width=0.48\textwidth]{Figures/comparative_superlative.jpeg}
%     \caption{An overview of aligned embedding spaces. (a) An example of alignment of semantic directions (i.e. plurality) in word embedding space. (b) An example of alignment of drug signatures across cell types in gene expression embedding space.}
%     \label{fig: Overview Schematic}
% \end{figure}


% More generally, aligned latent spaces are useful for tasks such as imputation \cite{jia2021deep}, image interpolation \cite{bojanowski2017optimizing},  and zero-shot learning \cite{}.  
% Hence, semantic shifts in the input space correspond to translations along the aligned direction in latent space.


% Recent work \cite{TheisAutoencoding} empirically demonstrated that under-parameterized variational autoencoders \cite{VAE} naturally align a single perturbation (corresponding to cell stimulation) across multiple cell types on gene expression data.  Further work \cite{COVIDAutoencoding} replicated this finding for over-parameterized leaky ReLU autoencoders for gene expression vectors of drug and cell type combinations from the connectivity map (CMap) \cite{CMap} (See Figure \ref{fig: Overview Schematic}b). 


% \subsection*{Our Contributions}

The main finding of this work is that autoencoders can produce aligned latent spaces by stretching along the top left singular vectors of the data.  The following are our contributions. 

\begin{enumerate}
    \item We prove that stretching along the top singular vectors of the data  leads to  alignment in the latent space.  We analyze the case of a mixture of Gaussians with unaligned major axes and prove that stretching along the top left singular vectors aligns these axes.  
    \item We prove that asymmetrically initialized linear autoencoders stretch along the top left singular vectors of the data, thereby producing aligned latent spaces.  We derive the stretching factor through a gradient flow analysis.  In a simplified setting, we prove that, under low rank initialization, non-linear autoencoders also stretch along the top left singular vectors of the data.  
    \item  We apply our theory to produce autoencoders on GloVe embeddings \cite{pennington2014glove} that strengthen alignment of meaningful semantic directions.  The resulting aligned latent spaces provide an improvement on word analogy tasks. We lastly apply our theory to produce autoencoders that align drug signatures across cell types on gene expression data from CMap~\cite{CMap}.  
\end{enumerate}


==> Alignment via Over-parameterized Autoencoders/sections/preliminaries.tex <==
\label{sec: Preliminaries}

We begin with the training setup for vanilla autoencoders.  

\begin{definition}[Autoencoding]  Given a dataset $X \in \mathbb{R}^{d \times n}$ with $n$ training examples and neural network $f_{\theta}(x): \mathbb{R}^{d} \to \mathbb{R}^{d}$ with parameters $\theta \in \mathbb{R}^{p}$, gradient descent is used to solve
\begin{align}
    \label{eq: Autoencoder Loss} 
    \argmin_{\theta \in \mathbb{R}^{p}}  \mathcal{L}(X, \theta), ~~ \text{where} ~~ \mathcal{L}(X, \theta) =  \sum_{i=1}^{n} \| x^{(i)} - f(x^{(i)})\|_2^2, ~ 
\end{align}
 where $x^{(i)}$ denotes the $i$\textsuperscript{th} column of $X$.  
\end{definition}

In this work, we will reference the following spectral initialization scheme used in \cite{ImplictRegularizationBach, Saxe2014, Saxe2019}. 
\begin{definition}[Spectral Initialization]  
\label{def: Spectral Initialization}
Let $f(x) = A B x$ denote a linear autoencoder with $x \in \mathbb{R}^{d}$, $A \in \mathbb{R}^{d \times k}$, and $B \in \mathbb{R}^{k \times d}$.  We assume gradient descent is used to solve Eq. \eqref{eq: Autoencoder Loss} on dataset $X$ and let $A^{(0)}, B^{(0)}$ denote the parameters at initialization.  The \textbf{spectral initialization} corresponds to $A^{(0)} = U_X \Sigma_A^{(0)} U_X^T,  B^{(0)} = U_X \Sigma_B^{(0)} U_X^T$ where $U_X$ denotes the left singular vectors of $X$ and $\Sigma_A^{(0)}, \Sigma_B^{(0)}$ are positive, semi-definite diagonal matrices.   
\end{definition}

The spectral initialization scheme is commonly used to understand training dynamics in neural networks.  Assuming \textit{symmetric} spectral initialization (i.e. $\Sigma_A^{(0)} = \Sigma_B^{(0)}$)  and that the rank of $A^{(0)}$ equals the rank of $X$, solving Eq. \eqref{eq: Autoencoder Loss} with gradient flow (i.e. gradient descent with infinitesimal step size) recovers the well-known result that linear autoencoders project onto the subspace spanned by the top principal components of the data \cite{AutoencodersPCAVectors}.  
% For analyzing non-linear autoencoders, we use the following low-rank initialization scheme \cite{RadhakrishnanOPAMemory}.  

% \begin{definition}[Low Rank Initialization]  
% \label{def: Low Rank Initialization}
% Let $f(x) = A \phi(B x)$ denote a nonlinear autoencoder with $x \in \mathbb{R}^{d}$, $A \in \mathbb{R}^{d \times k}$, $B \in \mathbb{R}^{k \times d}$, and $\phi$ an elementwise nonlinearity.  We assume gradient descent is used to solve Eq. \eqref{eq: Autoencoder Loss} on dataset $X$ and let $A^{(0)}, B^{(0)}$ denote the parameters at initialization.  The \textbf{low rank initialization} corresponds to $A^{(0)} = \sum_{i=1}^{n} x^{(i)} {a^{(i)}}^T,  B^{(0)} = \sum_{i=1}^{n}b^{(i)} {x^{(i)}}^T$ where $a^{(i)}, b^{(i)} \in \mathbb{R}^{k}$.  
% \end{definition}

% The low rank initialization remains invariant throughout training with gradient flow, as shown in \cite{RadhakrishnanOPAMemory}.  Under this scheme, only the vectors $a^{(i)}, b^{(i)}$ are updated and \cite{RadhakrishnanOPAMemory} uses this to analyze over-parameterized autoencoders trained on single examples.  


==> Alignment via Over-parameterized Autoencoders/sections/related_work.tex <==
\label{sec: Related Work}
Prior work \cite{TheisAutoencoding} demonstrated empirically that variational autoencoders \cite{VAE} can align the effect of perturbations across multiple cell types in single-cell gene expression data. In particular, the work demonstrated that under-parameterized, non-linear autoencoders automatically align the effect of stimulating cells by a single perturbation (IFN-$\beta$) in the latent space.  Follow-up work \cite{COVIDAutoencoding} demonstrated that over-parameterized 1-hidden layer autoencoders with leaky ReLU \cite{LeakyReLU} activation align the effect of multiple perturbations between cell types from the connectivity map (CMap) \cite{CMap}.  In this work, we prove that over-parameterized, 1-hidden layer autoencoders produce aligned latent spaces by stretching along the top left singular vectors of the data.  

Several recent works \cite{belkin2019reconciling, TwoModelsDoubleDescent, DeepDoubleDescent} study the behavior of over-parameterized neural networks in supervised learning.  While there are infinitely many interpolating solutions in the over-parameterized regime, these works demonstrated that an implicit bias through training encourages solutions that generalize.  Further works \cite{IdentityCrisis, RadhakrishnanOPAMemorization, RadhakrishnanOPAMemory} characterized the implicit bias of over-parameterized autoencoders in unsupervised settings.  In particular, \cite{RadhakrishnanOPAMemory, RadhakrishnanOPAMemorization} demonstrated that over-parameterized autoencoders learn solutions that are contractive around the training examples.  These works, however, did not analyze the latent space produced by over-parameterized autoencoders.  

% For our proofs of alignment in non-linear autoencoders, we follow the initialization used in \cite{RadhakrishnanOPAMemory}, but we analyze networks with ReLU (non-smooth) activation \textcolor{red}{Is this last sentence required?}.


It is well-known that linear autoencoders under a balanced spectral initialization \cite{Balancedness, Saxe2014, Saxe2019, ImplictRegularizationBach} learn the subspace spanned by the top principal components of the data \cite{AutoencodingPCA, AutoencodersPCAVectors}.  In this work, we analyze over-parameterized linear autoencoders under an asymmetric spectral initialization, i.e. one layer is initialized at 0 and the other is initialized using a matrix polynomial in the data.  Importantly, unlike prior spectral initialization analyses, our asymmetric initialization is easy to compute in practice.   In order to derive the solution at the end of training in linear autoencoders under spectral initialization, we use a gradient flow analysis, i.e. gradient descent with infinitesimal step size  \cite{ImplictRegularizationBach, RadhakrishnanOPAMemory, BalancednessJasonLee}. 

% Lastly, in this paper we consider finite-width neural networks.  Indeed, a neural tangent kernel (NTK) \cite{NTKJacot} analysis is not readily applicable for extracting embeddings for infinite-width neural networks, since the embedding from the NTK is an identity transformation of the original data~\cite{GregYangFeatureLearning}. \textcolor{red}{I don't know what you want to say with this.}

% Prior work \cite{TheisAutoencoding} demonstrated empirically that variational autoencoders \cite{VAE} can align the effect of perturbations across multiple cell types in single cell gene expression data. In particular, this work demonstrated that under-parameterized, non-linear autoencoders automatically align the effect of stimulating cells by a single perturbation (IFN-$\beta$) in the latent space.  Follow up work, \cite{COVIDAutoencoding}, demonstrated that over-parameterized 1 hidden layer autoencoders with leaky ReLU \cite{LeakyReLU} activation align the effect of multiple perturbations between cell types from the connectivity map (CMap) \cite{CMap}.  In this work, we prove that this alignment phenomenon is due to stretching along the top left singular vectors of the data.  We additionally prove that over-parameterized, 1 hidden layer, linear autoencoders re-create this alignment phenomenon when using an asymmetric initialization for the layers.  

% Several recent works \cite{belkin2019reconciling, TwoModelsDoubleDescent, DeepDoubleDescent} establish the benefits of using over-parameterized neural networks, i.e. those capable of achieving zero training error, in supervised learning.  In particular, while there are infinitely many interpolating solutions in the over-parameterized setting, these works demonstrate that there is an implicit bias through training that leads to solutions that generalize.  While previous works focused on the supervised setting, \cite{IdentityCrisis, RadhakrishnanOPAMemorization, RadhakrishnanOPAMemory} characterize the implicit bias of over-parameterized autoencoders.  In particular, \cite{RadhakrishnanOPAMemory, RadhakrishnanOPAMemorization} demonstrate that over-parameterized autoencoders learn solutions that are contractive around the training examples.  These works, however, focused on autoencoders initialized near zero and did not analyze the latent space produced by over-parameterized autoencoders.  For our proofs of alignment in non-linear autoencoders, we follow the initialization used in \cite{RadhakrishnanOPAMemory}, but we analyze networks with ReLU (non-smooth) activation.


% It is well known that linear autoencoders under a spectral initialization \cite{Saxe2014, Saxe2019, ImplictRegularizationBach} learn the subspace spanned by the top principal components of the data \cite{AutoencodingPCA}.  Using the singular vectors of the layers for a 1 hidden layer linear autoencoder under the spectral initialization also recovers the loading vectors  \cite{AutoencodersPCAVectors}.  In this work, we analyze over-parameterized linear autoencoders under an asymmetric spectral initialization, i.e. one layer is initialized at 0 and the other is initialized using a matrix polynomial in the data.  Importantly, unlike the case for the prior spectral initialization analyses, our asymmetric initialization is easy to compute in practice.  Our asymmetric initialization produces a different embedding of the data than that of prior spectral initialization analyses.  In order to derive the solution at the end of training in linear autoencoders under spectral initialization, we use a gradient flow analysis, i.e. gradient descent with infinitesimal step size  \cite{ImplictRegularizationBach, RadhakrishnanOPAMemory, BalancednessJasonLee}. 

% Lastly, in this paper we consider finite width neural networks.  Indeed, a neural tangent kernel (NTK) \cite{NTKJacot} analysis is not readily applicable for extracting embeddings for infinite width neural networks since the embedding from the NTK is similar to an identity transformation of the original data \cite{GregYangFeatureLearning}. 

==> Alignment via Over-parameterized Autoencoders/sections/stretching_section/2d_gaussian_ommitted_arithmetic.tex <==
Define the following helper variables:
$$a = \alpha + \beta, \quad b = \alpha - \beta, \quad  x = \sqrt{c^2 + 4} + c, \quad  y = \sqrt{c^2 + 4} - c, z = a^2 + b^2, r=\alpha^2 + \beta^2, s = \alpha^2 - \beta^2$$
Note the following:
\begin{align*}
    z &= 2(\alpha^2 + \beta^2)\\
    z^2 &= 4(\alpha^2 + \beta^2)^2\\
    x + y &= 2 \sqrt{c^2 + 4}\\
    xy &= 4\\
    x^2 + y^2 &= 4(c^2 + 2)\\
    ab &= \alpha^2 - \beta^2\\
    abz &= 2(\alpha^4 - \beta^4)\\
    a^2b^2 &= (\alpha^2 - \beta^2)^2
\end{align*}
    
Then we have that 
\begin{align*}
    E[B] &= \begin{bmatrix}
    a & b\\
    b & a
    \end{bmatrix}, q_{\Sigma_1} = \begin{bmatrix} 2 \\ x \end{bmatrix}, q_{\Sigma_2} = \begin{bmatrix} 2 \\ y \end{bmatrix}\\
    E[Bq_{\Sigma_1}] &= \begin{bmatrix} 2a + bx \\ 2b + ax \end{bmatrix} \quad E[Bq_{\Sigma_2}] = \begin{bmatrix} 2a + by \\ 2b + ay \end{bmatrix}\\
\end{align*}
We first take the dot product:
\begin{align*}
     E[Bq_{\Sigma_1}]^T E[Bq_{\Sigma_2}] &=  4a^2 + 2aby + 2abx + b^2xy + 4b^2 + 2bay + 2bax + a^2xy\\
     &= 8z + 4ab(x+y)\\
     &= 8(2(\alpha^2 + \beta^2) + (\alpha^2 - \beta^2) \sqrt{c^2 + 4})
\end{align*}
We then take the norms:
\begin{align*}
    ||E[Bq_{\Sigma_1}]||_2^2 &= (2a+bx)^2 + (2b + ax)^2\\
    &= 4a^2 + 4bax + b^2x^2 + 4b^2 + 4bax + a^2x^2\\
    &= 4(a^2 + b^2) + 8bax + x^2(a^2 + b^2)\\
    &= (x^2 + 4)z + 8abx\\
    ||E[Bq_{\Sigma_2}]||_2^2 &= (y^2 + 4)z + 8aby\\
     ||E[Bq_{\Sigma_1}]||_2^2 ||E[Bq_{\Sigma_2}]||_2^2 &= ((x^2 + 4)z + 8abx)((y^2 + 4)z + 8aby)\\
     &= (x^2+4)(y^2+4)z^2 + (x^2+4)z*8aby + (y^2+4)z * 8abx + 64a^2b^2xy\\
     &= (x^2+4)(y^2+4)z^2  + 8abz(y(x^2+4) + x(y^2+4)) + 256a^2b^2\\
     (x^2+4)(y^2+4)z^2 &= (x^2y^2 + 4x^2 + 4y^2 + 16)z^2\\
     &= (32 + 4(x^2 + y^2))(z^2)\\
     &= (32 + 16(c^2+2))(z^2)\\
     &= 4(64 + 16c^2)(\alpha^2 + \beta^2)^2\\
     &= 64(4 + c^2)(\alpha^2 + \beta^2)^2\\
     8abz(y(x^2+4) + x(y^2+4)) &= 8abz(x^2y + 4y + xy^2 + 4x)\\
     &= 8abz(4x + 4y + 4y + 4x)\\
     &= 64abz(x+y)\\
     &= 256(\alpha^4 - \beta^4)(\sqrt{c^2 + 4})\\
     256a^2b^2 &= 256(\alpha^2 - \beta^2)^2\\
     ||E[Bq_{\Sigma_1}]||_2^2 ||E[Bq_{\Sigma_2}]||_2^2 &= 64(4 + c^2)(\alpha^2 + \beta^2)^2 + 256(\alpha^4 - \beta^4)(\sqrt{c^2 + 4}) + 256(\alpha^2 - \beta^2)^2\\
     &= 64\left((4 + c^2)(\alpha^2 + \beta^2)^2 + 4(\alpha^4 - \beta^4)(\sqrt{c^2 + 4}) + 4(\alpha^2 - \beta^2)^2 \right)\\
     &= 64\left( (c^2+4)r^2 + 4rs\sqrt{c^2+4} + 4s^2 \right)\\
     &= 64(\sqrt{c^2 + 4}r + 2s)^2\\
     &= 64\left(\sqrt{c^2+4}(\alpha^2 + \beta^2) + 2(\alpha^2 - \beta^2)\right)^2\\
\end{align*}

Then combining the two we have:
\begin{align*}
    \frac{E[Bq_{\Sigma_1}]^T E[Bq_{\Sigma_2}]}{\sqrt{||E[Bq_{\Sigma_1}]||_2^2 ||E[Bq_{\Sigma_2}]||_2^2}} &= \frac{2(\alpha^2 + \beta^2) + (\alpha^2 - \beta^2) \sqrt{c^2 + 4}}{(\alpha^2 + \beta^2)\sqrt{c^2+4} + 2(\alpha^2 - \beta^2)}\\
    &=  \frac{2 + \gamma \sqrt{c^2 + 4}}{2\gamma + \sqrt{c^2 + 4}} , \quad \gamma = \frac{(\alpha^2 - \beta^2)}{(\alpha^2 + \beta^2)}
\end{align*}


==> Alignment via Over-parameterized Autoencoders/sections/stretching_section/2d_gaussian_stretch_previous_draft.tex <==
\begin{lemma}
Consider the setting in Lemma \ref{lemma: XXT}, where $X_1, X_2 \in \mathbb{R}^{2 \times n}$. Let $X_1 \sim \mathcal{N}(e_1, \Sigma_1), X_2 \sim \mathcal{N}(e_2, \Sigma_2)$. Let $v = [1,1]^T$, $\hat{v} = \frac{[1,1]^T}{\sqrt{2}}$, and
$$D_1 = \begin{bmatrix} c & 0 \\ 0 & 1 \end{bmatrix}, \Sigma_1 = D_1 + vv^T = D_1 + J$$
$$D_2 = \begin{bmatrix} 1 & 0 \\ 0 & c \end{bmatrix}, \Sigma_2 = D_2 + vv^T = D_2 + J$$

Then before autoencoding, the cosine distance between the first principal directions of $X_1$ and $X_2$ is
$$ \cos(\theta_c) = \frac{2}{\sqrt{4 + (c-1)^2}}$$
and the cosine distance between the principal directions of the linearly autoencoded $X_1, X_2$, having set $A^{(0)} = 0, B^{(0)} = \left(\frac{1}{n}XX^T\right)^k$, is
$$\cos(\theta_c') = \frac{\alpha^2(c+5) - \beta^2(c+1)}{\sqrt{(\alpha^2(c+5) - \beta^2(c+1))^2 + 4 \alpha^2 \beta^2 (c-1)^2}}$$
for
$$\alpha = (\Sigma_B)_1 = \sqrt{\frac{(c+6)^{2k}}{2} + \sqrt{1 + \frac{(c+6)^{4k}}{4}}}, \beta = (\Sigma_B)_2 = \sqrt{\frac{(2+c)^{2}}{2} + \sqrt{1 + \frac{(2+c)^{4}}{4}}}$$

Moreover, 
$$cos(\theta_c) < cos(\theta_c'), \quad \forall c> 1$$ 
\textcolor{blue}{Saachi: This last statement is just from the plot for now}

\end{lemma}

Let $\lambda_i$ be the $i$th eigenvalue of $XX^T$. By Theorem \ref{theorem: two layer linear autoencoder}, if we initialize $A^{(0)}=0$ and  $B^{(0)} = \frac{1}{n} (XX^T)^k = U_X \Sigma_B U_X^T$, then after gradient descent we have:
$$B = U_X \Sigma_B U_X^T, (\Sigma_B)_i = \sqrt{\frac{\lambda_i^{2}}{2} + \sqrt{1 + \frac{\lambda_i^{4}}{4}}}$$

For our particular setting, from Theorem \ref{lemma: XXT},  we can calculate the expected value of $B^{(0)}$
$$E[B^{(0)}] = \mathbb{E}_{X_1, X_2}[\frac{1}{n} XX^T] = (2+c) I + 2 J = (2+c) I + 4\hat{v}\hat{v}^T$$
with eigenvectors $\hat{v}$ and $\hat{u} = [1, -1]^T/\sqrt{2}$ with eigenvalues:
$\lambda_1 = (c + 6), \lambda_2 = (2+c)$.

Then we have 

\noindent\fbox{%
    \parbox{\textwidth}{%
$$\alpha = (\Sigma_B)_1 = \sqrt{\frac{(c+6)^{2k}}{2} + \sqrt{1 + \frac{(c+6)^{4k}}{4}}}, \beta = (\Sigma_B)_2 = \sqrt{\frac{(2+c)^{2}}{2} + \sqrt{1 + \frac{(2+c)^{4}}{4}}}$$
and eigenvectors $\hat{v}$ and $\hat{u}$.
    }%
}
Then let $U_X$ be:
$$U_X = \begin{bmatrix} \hat{v} & \hat{u} \end{bmatrix} = \frac{1}{\sqrt{2}}\begin{bmatrix}1 & 1 \\ 1 & -1\end{bmatrix}$$

Then we have:
\begin{align*}B &= \frac{1}{2}
\begin{bmatrix}1 & 1 \\ 1 & -1\end{bmatrix}
\begin{bmatrix} \alpha & 0 \\ 0 & \beta \end{bmatrix}
\begin{bmatrix}1 & 1 \\ 1 & -1\end{bmatrix}\\
&= \frac{1}{2}
\begin{bmatrix}\alpha & \beta \\ \alpha & -\beta\end{bmatrix}
\begin{bmatrix}1 & 1 \\ 1 & -1\end{bmatrix}\\
&=  \frac{1}{2} \begin{bmatrix} \alpha + \beta & \alpha - \beta \\ \alpha - \beta & \alpha + \beta\end{bmatrix}\\
&= \frac{1}{2}(\alpha J + \beta \tilde{J})
\end{align*}
Where 
$$\tilde{J} = \begin{bmatrix} 1 & -1 \\ -1 & 1 \end{bmatrix}$$

First note that:
$$JJ = 2J, \quad \tilde{J} J = 0, \quad  JD_iJ = (c+1)J, \quad \tilde{J}D_i\tilde{J} = (c+1) \tilde{J}$$
$$\tilde{J}D_1J + JD_1\tilde{J} = (2c-2)\text{diag}([1, -1])$$
$$\tilde{J}D_2J + JD_2\tilde{J} = (2c-2)\text{diag}([-1, 1])$$


Then what is the expected covariance of the centered $X_i$ after autoencoding?:
\begin{align*}
Cov(BX_i) = E&[(BX_i - E[BX_i])(BX_i - E[BX_i])^T]\\
&= B\Sigma_1B^T\\
&= \frac{1}{4} (\alpha J + \beta \tilde{J}) (D_i + J) (\alpha J + \beta \tilde{J})\\
&= \frac{1}{4} (\alpha J D_i + \beta \tilde{J} D_i + \alpha J J + \beta \tilde{J} J) (\alpha J + \beta \tilde{J})\\
&= \frac{1}{4} (\alpha J D_i + \beta \tilde{J} D_i + 2 \alpha J) (\alpha J + \beta \tilde{J})\\
&= \frac{1}{4} (\alpha^2 J D_i J + \beta \alpha \tilde{J} D_i J + 2 \alpha^2 J J + \alpha \beta J D_i \tilde{J} + \beta ^2\tilde{J} D_i \tilde{J} + 2 \alpha \beta J  \tilde{J})\\
&= \frac{1}{4}(\alpha^2 (c+1) J + \alpha \beta(\tilde{J} D_i J + J D_i \tilde{J}) + 4 \alpha^2 J + \beta^2 (c+1) \tilde{J})\\
\end{align*}
For $X_1$ this is:
\begin{align*}
Cov(BX_1)   &= \frac{1}{4} (\alpha^2 (c+5)J + \alpha \beta (2c-2)\text{diag}([1, -1])  + \beta^2(c+1) \tilde{J})\\
&= \frac{1}{4} \begin{bmatrix} 
\alpha^2(c+5) + 2\alpha \beta(c-1) + \beta^2(c+1) & \alpha^2(c+5) - \beta^2(c+1)\\
 \alpha^2(c+5) - \beta^2(c+1) & \alpha^2(c+5) - 2\alpha \beta(c-1) + \beta^2(c+1)
\end{bmatrix}
\end{align*}
And for $X_2$ we simply flip to get:
\begin{align*}
Cov(BX_2) &= \frac{1}{4} \begin{bmatrix} 
\alpha^2(c+5)  - 2\alpha \beta(c-1) + \beta^2(c+1) & \alpha^2(c+5) - \beta^2(c+1)\\
 \alpha^2(c+5) - \beta^2(c+1) & \alpha^2(c+5) + 2\alpha \beta(c-1) + \beta^2(c+1)
\end{bmatrix}
\end{align*}

% use formula from here to get eigenvectors and values http://scipp.ucsc.edu/~haber/ph116A/diag2x2_11.pdf

Let $r = \alpha^2(c+5)$, $s = 2\alpha \beta(c-1)$, $t = \beta^2(c+1)$. Then the above matrices have the form:
$$
Cov(BX_1) = \begin{bmatrix}
r + s + t & r-t\\
r-t & r- s + t
\end{bmatrix}
$$
$$
Cov(BX_2) = \begin{bmatrix}
r - s + t & r-t\\
r-t & r + s + t
\end{bmatrix}
$$

$Cov(BX_1)$ has eigenvalues:
\begin{align*}
    \lambda(Cov(BX_1)) = r + t \pm \sqrt{s^2 + (r-t)^2}
\end{align*}
and eigenvectors:
\begin{align*}
    (q_{(BX_1)})_1 = \begin{bmatrix} r - t \\ \sqrt{s^2 + (r-t)^2} + s\end{bmatrix}, \quad
    (q_{(BX_1)})_2 = \begin{bmatrix} r - t \\ -\sqrt{s^2 + (r-t)^2} + s\end{bmatrix}
\end{align*}

and similarly $Cov(BX_2)$ has eigenvalues:
\begin{align*}
    \lambda(Cov(BX_1)) = r + t \pm \sqrt{s^2 + (r-t)^2}
\end{align*}
and eigenvectors:
\begin{align*}
    (q_{(BX_1)})_1 = \begin{bmatrix} r - t \\ \sqrt{s^2 + (r-t)^2} - s\end{bmatrix}, \quad
    (q_{(BX_1)})_2 = \begin{bmatrix} r - t \\ -\sqrt{s^2 + (r-t)^2} - s\end{bmatrix}
\end{align*}

We want the cosine distance between $(q_{(BX_1)})_1$ and $(q_{(BX_1)})_1$ is:
\begin{align*}
    (q_{(BX_1)})_1 \cdot (q_{(BX_1)})_2  &= (r-t)^2 + s^2 + (r-t)^2 - s^2\\
    &= 2 (r-t)^2\\
    ||(q_{(BX_1)})_1||_2^2 &= (r-t)^2 + s^2 + s^2 + (r-t)^2 +2s \sqrt{s^2 + (r-t)^2}\\
    &= 2(r-t)^2 + 2s^2 + 2s \sqrt{s^2 + (r-t)^2}\\
    ||(q_{(BX_1)})_2||_2^2 &= (r-t)^2 + s^2 + s^2 + (r-t)^2  - 2s \sqrt{s^2 + (r-t)^2}\\
    &= 2(r-t)^2 + 2s^2 - 2s \sqrt{s^2 + (r-t)^2}\\
    ||(q_{(BX_1)})_1||_2^2 ||(q_{(BX_1)})_2||_2^2 &= 4 (((r - t)^2 + s^2)^2 - s^2 (s^2 + (r-t)^2))\\
    &= 4((r-t)^2 + s^2)(r-t)^2\\
    \cos(\theta') &= \frac{(r-t)}{\sqrt{((r-t)^2 + s^2)}}\\
    &= \frac{\alpha^2(c+5) - \beta^2(c+1)}{\sqrt{(\alpha^2(c+5) - \beta^2(c+1))^2 + 4 \alpha^2 \beta^2 (c-1)^2}}
\end{align*}
The original eigenvalues of $\Sigma_1 = \begin{bmatrix} c+1 & 1 \\ 1 & 2 \end{bmatrix}$ and $\Sigma_2 =  \begin{bmatrix} 2 & 1 \\ 1 & c+1 \end{bmatrix}$ 
\begin{align*}
    \lambda &= \frac{1}{2} (c+3 \pm \sqrt{(c-1)^2 + 4}\\
\end{align*}
With eigenvectors:
$$(q_{(\Sigma_1})_1 = \begin{bmatrix} 2 \\ 1 - c + \sqrt{(c-1)^2 + 4}  \end{bmatrix},
(q_{(\Sigma_1})_2 = \begin{bmatrix} 2 \\ 1 - c - \sqrt{(c-1)^2 + 4}  \end{bmatrix}$$
$$(q_{(\Sigma_2})_1 = \begin{bmatrix} 2 \\ c-1 + \sqrt{(c-1)^2 + 4}  \end{bmatrix},
(q_{(\Sigma_2})_2 = \begin{bmatrix} 2 \\ c-1 - \sqrt{(c-1)^2 + 4}  \end{bmatrix}$$

We again find the cosine distance:
\begin{align*}
    (q_{(\Sigma_1})_1 \cdot (q_{(\Sigma_1})_2 &= 4 + (c-1)^2 + 4 - (c-1)^2\\
    &= 8\\
    || (q_{(\Sigma_1})_1 ||_2^2 &= 4 + (c-1)^2 + (c-1)^2 + 4 - 2 (c-1) \sqrt{(c-1)^2 + 4}\\
    &= 8 + 2(c-1)^2 - 2 (c-1) \sqrt{(c-1)^2 + 4}\\
    || (q_{(\Sigma_1})_2 ||_2^2 &= 4 + (c-1)^2 + (c-1)^2 + 4 + 2 (c-1) \sqrt{(c-1)^2 + 4}\\
    &= 8 + 2(c-1)^2 + 2 (c-1) \sqrt{(c-1)^2 + 4}\\
    || (q_{(\Sigma_1})_1 ||_2^2 || (q_{(\Sigma_1})_2 ||_2^2 &= 4(4 + (c-1)^2)^2 - 4(c-1)^2 ((c-1)^2 + 4)\\
    &= 4(4 + (c-1)^2)(4)\\
    \cos(\theta) &= \frac{2}{\sqrt{4 + (c-1)^2}}
\end{align*}
Thus our before and after cosine distances of the major principal directions are 

\noindent\fbox{%
    \parbox{\textwidth}{%
    $$ \cos(\theta) = \frac{2}{\sqrt{4 + (c-1)^2}}, \quad \cos(\theta') = \frac{\alpha^2(c+5) - \beta^2(c+1)}{\sqrt{(\alpha^2(c+5) - \beta^2(c+1))^2 + 4 \alpha^2 \beta^2 (c-1)^2}}$$
    for
    $$\alpha = (\Sigma_B)_1 = \sqrt{\frac{(c+6)^{2k}}{2} + \sqrt{1 + \frac{(c+6)^{4k}}{4}}}, \beta = (\Sigma_B)_2 = \sqrt{\frac{(2+c)^{2}}{2} + \sqrt{1 + \frac{(2+c)^{4}}{4}}}$$
    }%
}

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{Figures/translation_alignment_plot_cosine_sims.png}
    \caption{We plot the cosine distance (original and autoencoded for different polynomial $k$) between the top principal direction of the two gaussians for increasing values of $c$.
}
    \label{fig:Gaussian 2D alignment}
\end{figure}


==> Alignment via Over-parameterized Autoencoders/sections/stretching_section/2d_gaussian_stretching.tex <==
% In Corollary \ref{corollary: Stretching along means}, we found that the top singular vector for a mixture of Gaussians will point in the direction of the average of the means.  We now show that stretching along this direction can yield alignment of the major axes of individual Gaussians in the mixture.  


We now consider a setting with two Gaussians in $\mathbb{R}^2$ and use Lemma \ref{lemma: Stretching along means} to prove that stretching this mixture of Gaussians along the average of the means will align the major axes of the individual Gaussians (proof in Appendix \ref{appendix: two gaussians}).
\begin{corollary}
\label{corollary: two gaussians}
Let $X_1, X_2 \in \mathbb{R}^{2 \times n}$ with $X_1^{(i)} \sim \mathcal{N}(e_1, \Sigma_1), X_2^{(i)} \sim \mathcal{N}(e_2, \Sigma_2)$ for $i \in [n]$ where $e_1=[1,0]^T$, $e_2=[0,1]^T$, and $J$ is the all ones matrix.  Let $X = [ X_1 | X_2 ]$, and
$$D_1 = \begin{bmatrix} c+1 & 0 \\ 0 & 1 \end{bmatrix}, \Sigma_1 = D_1 + J ~~ ; ~~ D_2 = \begin{bmatrix} 1 & 0 \\ 0 & c+1 \end{bmatrix}, \Sigma_2 = D_2 + J.$$
Then $\EE[XX^T]$ has eigenvectors $u_1=\frac{1}{\sqrt{2}}[1,1]^T$ and  $u_2=\frac{1}{\sqrt{2}}[1,-1]^T$.
% We train a linear autoencoder on $X$, initialized such that $A^{(0)} = 0$ and $B^{(0)} = \frac{1}{n}XX^T$. 

Consider the embedding $BX$, where $B \in \mathbb{R}^{d \times d}$ has eigenvectors $u_1$ and $u_2$ and corresponding eigenvalues $\alpha$ and $\beta$ where $\alpha^2 > \beta^2$. Let $q_{\Sigma_1}$ and $q_{\Sigma_2}$ be the top eigenvectors of $\Sigma_1$ and $\Sigma_2$. Then the cosine similarity of $q_{\Sigma_1}$ and $q_{\Sigma_2}$ before and after embedding with $B$ is:
$$ \cos(q_{\Sigma_1}, q_{\Sigma_2}) = \frac{2}{\sqrt{4 + c^2}}, \quad \quad  \cos(Bq_{\Sigma_1}, Bq_{\Sigma_2}) = \frac{2 + \gamma \sqrt{c^2 + 4}}{2\gamma + \sqrt{c^2 + 4}}$$
for $\gamma = \frac{(\alpha^2 - \beta^2)}{(\alpha^2 + \beta^2)}$.
Moreover, $\cos(Bq_{\Sigma_1}, Bq_{\Sigma_2})>  \cos(q_{\Sigma_1}, q_{\Sigma_2}).$
\end{corollary}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{Figures/translation_alignment_before_ae.png}\hfill
%     \includegraphics[width=0.45\textwidth]{Figures/translation_alignment_after_ae.png}
%     \caption{Setting for translation alignment in Section \ref{translation_alignment} before autoencoding (left) and after autoencoding (right). We see that stretch along $[1,1]^T$ makes the principal directions of the two distributions more aligned. }
%     \label{fig:Gaussian 2D alignment}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=1\textwidth]{Figures/GaussianAlignment.pdf}
%     \caption{Alignment of the major axes of Gaussians in a mixture, $X$, increases after stretching along the top singular vector of $X$. (a) Two Gaussians with major axes that are nearly orthogonal.  (b) Alignment of the major axes after stretching along the top singular vector of $X$.}
%     \label{fig:Gaussian 2D alignment}
% \end{figure}
% Setting for translation alignment in Corollary \ref{corollary: two gaussians} before autoencoding (a) and after autoencoding (b). We see that stretch along $[1,1]^T$ makes the principal directions of the two distributions more aligned.

Thus, if $B$ stretches along the top left singular vectors of $X$, then the major axes of individual Gaussians in the mixture become more aligned.  As is shown by the following corollary, setting $B = (\frac{1}{n} XX^T)^k$, for some degree $k \geq 1$ leads to alignment (Proof in Appendix \ref{appendis: two gaussians with xxt}).

% setting $B$ to stretch along the top principal direction of the dataset, which here is the average of the means, will align the otherwise mostly orthogonal major axes for the individual Gaussians. 


\begin{corollary}
\label{corollary: two gaussians with xxt}
In the setting of Corollary \ref{corollary: two gaussians}, if $B = (\frac{1}{n}XX^T)^k$,  then as $n$ tends to infinity,
$$\cos(B q_{\Sigma_1}, B q_{\Sigma_2}) \xrightarrow{a.s} \frac{2 + \gamma \sqrt{c^2 + 4}}{2\gamma + \sqrt{c^2 + 4}} , \quad \gamma = \frac{(\alpha^2 - \beta^2)}{(\alpha^2 + \beta^2)}$$
for $\alpha = (c+7)^k, \beta = (c+3)^k$.  Moreover, as $k$ increases $\cos(B q_{\Sigma_1}, B q_{\Sigma_2})$ also increases. 
% Thus the alignment of $q_1$ and $q_2$ will increase after encoding with $B$. Moreover, encoding with higher degrees $k$ will increase alignment. 
\end{corollary}
\textbf{Remarks.} We empirically verify this result in Appendix \ref{appendis: two gaussians with xxt}. The above corollaries imply that stretching along the top singular vector of the data aligns the major axes of the individual Gaussians.  In general, however, the degree of alignment depends on how aligned each direction of interest is to the overall stretching direction. As a simple example, in the above setting, stretching instead along the major axis of one of the Gaussians would not significantly boost alignment. Indeed, the ideal direction, $v$, to stretch along is one where semantically meaningful directions are roughly equally aligned with $v$.   Consistent with the result of this section, we show in Section \ref{sec: Applications} that stretching along the top eigenvector of $XX^T$ leads to alignment of semantically meaningful directions on large datasets.  

% As discussed in this section, multiplication by a high degree polynomial in $XX^T$ can yield alignment of directions of interest in data.  However, inverting the map to recover the data in the original space is can be expensive on high dimensional datasets.  In the next section, we will show that asymmetrically initialized autoencoders can be trained using gradient descent to produce latent spaces that automatically stretch along the  top eigenvectors of the dataset.   

% \begin{lemma}
%     Let $B \in \mathbb{R}^{d \times d}$ be a positive semi-definite matrix such with eigendecomposition $B=U\Sigma_BU^T$, where $\lambda_i$ and $u_i$ are the ith eigenvalue and eigenvector of $B$. and let $q_1, q_2 \in \mathbb{R}^d$ be unit vectors. Furthermore, let $\cos \theta_i^{(j)} = q_i^Tu_j$ be the angle between $q_i$ and the $j$th eigenvector. Then the cosine similarity of the embedded $Bq_1$ and $Bq_2$ is
%     $$\cos \theta' = \frac{
%         \sum_{i=1}^d \lambda_i^2 \cos \theta_i^{(1)} \cos \theta_i^{(2)}
%         }{\sqrt{
%             \left(\sum_{i=1}^k \lambda_i^2 (\cos \theta_i^{(1)})^2\right)
%             \left(\sum_{i=1}^k \lambda_i^2 (\cos \theta_i^{(2)})^2\right)
%         }}$$
% \end{lemma}
% This Lemma can gives us a few insights on a asymmetrically initialized linear autoencoder might encode individual directions. Firstly, if $q_1$ and $q_2$ are roughly equally aligned with the top singular vectors  (i.e  $\cos \theta_i^{(1)} = \cos \theta_i^{(2)}$), then $\cos \theta'$ will be closer to 1 and the autoencoded directions will be more aligned. This setting is similar to the example in Corollary \ref{corollary: two gaussians}. However, in a case where each singular vector is exactly aligned with one of individual directions but not the other (consider the pathological case where $\cos \theta_i^{(1)} = \mathbf{1}\{i \text{ is even}\}, \cos \theta_i^{(2)} = \mathbf{1}\{i \text{ is odd}\}$), then $\cos \theta'$ will be close to 0.

% For a high enough degree linear autoencoder, we note that $\lambda_1\gg \lambda_{i\neq 1}$. In this case, assuming that neither $q_1$ or $q_2$ are exactly orthogonal to $u_1$ (which would result in entirely squashing autoencoded direction), $\cos \theta \approx \pm 1$, where the directions will be \textit{aligned}  or $\textit{anti-aligned}$ depending on the sign of $\cos \theta_1^{(1)} \cos \theta_1^{(2)}$. \todo{do we want to put some synthetic figure here showing these cases. like we could have something where its just $q_1 = e_1$, $q_2 = e_2$, and then show the different cases of what directions we stretch.}


==> Alignment via Over-parameterized Autoencoders/sections/stretching_section/stretching.tex <==
In this section, we will show that stretching along the top left singular vectors of the data can boost alignment along directions of interest.  We begin by using the power method \cite{TrefethenBau} to provide intuition as to why stretching along singular vectors of the data leads to alignment.  

\textbf{Intuition from the Power Method.} The power method \cite{TrefethenBau} provides a mechanism for producing trivial alignment of directions in data.  Namely, repeated multiplication of data $X  \in \mathbb{R}^{d \times n}$ by a polynomial in $XX^T$ will project the data onto the top eigenvector of $XX^T$.  In this setting, the embedded points will lie on a line and thus, the cosine similarity between the difference of pairs of unique points will be either $1$ (perfectly aligned) or $-1$ (perfectly anti-aligned).\footnote{The number of iterations needed to produce perfect alignment depends on the numerical precision.}

% \todo{do we want to put a footnote about precision and that you normally don't need too many iterations to saturate?}

Fully projecting the data onto this top eigenvector is undesirable since this projection is not invertible and thus, we cannot decode the embedding back to the original input space. However, a partial iteration of the power method using $XX^T$ will stretch along the top eigenvector of $XX^T$ while yielding an invertible map.  We will demonstrate that using the power method to partially stretch along this top eigenvector is beneficial for aligning meaningful directions.  We begin by proving that stretching along this top eigenvector aligns the major axes of Gaussians in a mixture model.  


% \textbf{Intuition from the Power Method.} The power method \cite{TrefethenBau} provides a mechanism for producing trivial alignment of directions in data.  Namely, repeated multiplication of data $X  \in \mathbb{R}^{d \times n}$ by a polynomial in $XX^T$, $P[XX^T]$, leads to a projection onto the top eigenvector of $XX^T$.  Hence, multiplication by $P[XX^T]$ will result in all data points lying on a line and the cosine similarity between the difference of pairs of unique points will always one of $\{-1, 1\}$.  A full projection onto this top eigenvector is undesirable though since we cannot invert the projection map, which is essential for imputation tasks.  

% On the other hand, a partial iteration of the power method using $XX^T$ will stretch along the top eigenvector of $XX^T$ while still yielding an invertible map.  We will demonstrate that using the power method to partially stretch along this top eigenvector can be beneficial for aligning meaningful directions in a number of settings.  As an example, we begin by proving that stretching along this top eigenvector leads to the alignment of the major axes of Gaussians in a mixture model.  

% We focus on establishing alignment between the major axes of a mixture of Gaussians after stretching along the left singular vectors of the data.  Under conditions on the covariance matrices of Gaussians in the mixture, we prove that the top singular vector of the data is the sum of means of the Gaussians.  We then show that stretching along this direction leads to improved alignment of the major axes.  For the case of two dimensional Gaussians, we quantify the increase in cosine similarity between the major axes.




\subsection{Identifying the Top Singular Vector of a Gaussian Mixture}
\input{sections/stretching_section/stretching_lemmas}


\subsection{Quantifying Alignment in Gaussian Mixture Models}
\input{sections/stretching_section/2d_gaussian_stretching}


==> Alignment via Over-parameterized Autoencoders/sections/stretching_section/stretching_lemmas.tex <==
% \textcolor{red}{Do we want this sentence?} As is shown by the data distribution of gene expression data from \cite{COVIDAutoencoding}, the mixture of Gaussians model serves as a useful setting for establishing alignment of drug signatures across cell types. 

We will first characterize the top eigenvector and eigenvalue of $XX^T$ drawn from a mixture of Gaussians, and then use this result to quantify the increase in alignment after stretching along this top eigenvector. To aid our analysis, we choose a simple setting where we can explicitly compute the eigenvectors and eigenvalues of $\frac{1}{n}XX^T$ as $n \to \infty$ (Proof in Appendix~\ref{appendix: stretching_lemma}).
% \begin{lemma}
% \label{lemma: stretching lemma}
% Let $X_j = \{x_i^{(j)}\}_{i=1}^{n}  \in \mathbb{R}^{d \times n}$ for $j \in [m]$ where $x_i^{(j)} \sim \mathcal{N}(\mu_j, \Sigma_j)$. Then, as $n \to \infty$,
% $$\frac{1}{n} XX^T  \xrightarrow{a.s} \EE[\frac{1}{n}XX^T] = \sum_{j=1}^m (\Sigma_j + \mu_j \mu_j^T).$$
% \end{lemma}


\begin{lemma}
\label{lemma: Stretching along means}

Let $X_j = \{x_i^{(j)}\}_{i=1}^{n}  \in \mathbb{R}^{d \times n}$ for $j \in [m]$, where $x_i^{(j)} \sim \mathcal{N}(\mu_j, \Sigma_j)$. Assume $\Sigma_j = D_j + \mu_j(\sum_{i\neq j} \mu_i)^T$, such that $\sum_{j=1}^m D_j = cI$. Then as $n \to \infty$, 
$$\frac{1}{n} XX^T \xrightarrow{a.s} \EE\left[\frac{1}{n}XX^T\right] = cI + \left(\sum_{j=1}^m \mu_j\right)\left(\sum_{j=1}^m \mu_j\right)^T $$
with top eigenvector $(\sum_{j=1}^m \mu_j)/||\sum_{j=1}^m \mu_j||_2$ with eigenvalue $c + ||(\sum_{j=1}^m \mu_j)||_2^2$ and remaining eigenvectors $\{u ~; ~ ||u||_2^2 = 1, u \perp (\sum_{j=1}^m \mu_j)\}$ with eigenvalue $c$. 
\end{lemma}

By Lemma \ref{lemma: Stretching along means}, multiplication by $\frac{1}{n}XX^T$  will stretch along the direction of the average of the means.  We next verify that stretching along this direction leads to an alignment of major axes in a mixture of Gaussians.  

% In the setting of Lemma \ref{lemma: stretching lemma}, let $m=2$ and let $\Sigma_1 = D_1 + \mu_1 \mu_2^T$ and let $\Sigma_2 = D_2 + \mu_2 \mu_1^T$, such that $D_1 + D_2 = cI$ for $c \in \mathbb{R}$ and $I$ the identity matrix. Then,
% $$\mathbb{E}_{X_1, X_2}[\frac{1}{n} XX^T] = cI + (\mu_1 + \mu_2)(\mu_1 + \mu_2)^T$$

% With eigenvectors $(\mu_1 + \mu_2)/||(\mu_1 + \mu_2)||_2$ (eigenvalue $c + ||\mu_1 + \mu_2||_2^2$) and $\{u | ||u||_2^2 = 1, u^T (\mu_1 + \mu_2) = 0\}$ with eigenvalue $c$. Here, linear autoencoding will stretch along the eigenvector $(\mu_1 + \mu_2)/||(\mu_1 + \mu_2)||_2$.  Lemma \ref{lemma: stretching lemma} is a special case of the above lemma, where $c = 1+c', d=2, \mu_1 = e_1, \mu_2 = e_2$.\\


==> Alignment via Over-parameterized Autoencoders/sections/stretching_section/stretching_prelude.tex <==
\begin{figure}
    \centering
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=.7\textwidth]{Figures/s3_original_2.pdf}
    \caption{Original Space}
    \end{subfigure}
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=.7\textwidth]{Figures/s3_aligned_2.pdf}
    \caption{Encoding increases alignment}
    \end{subfigure}
    %     \begin{subfigure}{0.32\textwidth}
    % \centering
    % \includegraphics[width=\textwidth]{Figures/s3_unaligned.pdf}
    % \caption{Encoding decreases alignment }
    % \end{subfigure}
    \caption{Embedding data from a Gaussian mixture via a linear transformation can lead to alignment of the major axes depending on the spectrum of the transformation.}
    \label{fig:s3_alignment}
\end{figure}

% We show the effects of aligning this dataset with several choices of $B$. Depending on the direction of $B$'s first singular vector (in red), the major axes of the Gaussians can become more or less aligned.

% Given a dataset $X \in \mathbb{R}^{d \times n}$, one way to manipulate the  representation of $X$ is by embedding $X$ into a different latent space via autoencoders.  Autoencoders are a standard method for producing a latent representation for a dataset $X$.  As is done in \cite{COVIDAutoencoding}, we analyze pre-activation embeddings from 1 hidden layer over-parameterized autoencoders, and so, $X$ is embedded as $BX$ for $B \in \mathbb{R}^{h \times d}$.  

We briefly provide intuition around how stretching data, $X$, via multiplication by a linear transformation, $B$, can lead to alignment.  We begin by formally defining alignment:  we say that two directions $q_1, q_2$ become more \textit{aligned} in the latent space if their cosine similarity (which we write as $\cos(q_1, q_2)$) is smaller than their cosine similarity after embedding, $\cos(Bq_1, Bq_2)$.  Naturally, the alignment of directions in the latent space depends on $B$, as is illustrated by the following lemma (proof in Appendix \ref{appendix: Alignment Intuition}). 

\begin{lemma}
\label{lemma: Alignment Intuition}
    Let $B \in \mathbb{R}^{h \times d}$ have singular value decomposition $B=U\Sigma_BV^T$, where $\sigma_i$ and $v_i$ are the i\textsuperscript{th} singular value and right singular vector of $B$. Let $q_1, q_2 \in \mathbb{R}^d$ be unit vectors. Then,
    $$\cos(Bq_1, Bq_2) = \frac{
        \sum_{i=1}^d \sigma_i^2 \cos(q_1, v_i) \cos(q_2, v_i)
        }{\sqrt{
            \left(\sum_{i=1}^d \sigma_i^2 (\cos(q_1, v_i) ^2\right)
            \left(\sum_{i=1}^d \sigma_i^2 (\cos(q_2, v_i)^2\right)
        }}.$$
\end{lemma}

Lemma \ref{lemma: Alignment Intuition} demonstrates that the spectrum of $B$ governs whether two directions become more aligned.  For example, if $\sigma_1$ is much larger than $\sigma_i$ for $i > 1$ and the top eigenvector of $B$ has roughly similar cosine similarity between the two directions (i.e $\cos (q_1, v_1) \approx \cos(q_2, v_1)$), then $q_1$ and $q_2$ will become more aligned in the latent space.  In Figure \ref{fig:s3_alignment}, we give an example of a matrix $B$ that aligns the major axes of multivariate Gaussians by stretching along the direction $[1, 1]^T$.  

In this work, we identify a class of matrices $B$ that provably boost alignment for directions of interest.  We begin with a characterization of such $B$ for Gaussian mixture models in the next section. 

%  On the other hand, if  $\cos \theta_i^{(1)}$ and $\cos \theta_i^{(2)}$, then the vectors can become more orthogonal or even anti-aligned.


% 
% Consider the mixture of Gaussians in Figure TODO, for which the major axes of the individual Gaussians are nearly orthogonal to each other.  In this setting, we say that the embedding $BX$ is \textit{aligned} if the resulting major axes become nearly parallel. To characterize alignment of the representation $BX$, we analyze how the cosine similarity of two directions changes after multiplication by $B$.



% In Figure TODO, we revisit the example of two gaussians with largely orthogonal major axes...



% This setting is similar to the example in Corollary \ref{corollary: two gaussians}. However, in a case where each singular vector is exactly aligned with one of individual directions but not the other (consider the pathological case where $\cos \theta_i^{(1)} = \mathbf{1}\{i \text{ is even}\}, \cos \theta_i^{(2)} = \mathbf{1}\{i \text{ is odd}\}$), then $\cos \theta'$ will be close to 0.

% For a high enough degree linear autoencoder, we note that $\lambda_1\gg \lambda_{i\neq 1}$. In this case, assuming that neither $q_1$ or $q_2$ are exactly orthogonal to $u_1$ (which would result in entirely squashing autoencoded direction), $\cos \theta \approx \pm 1$, where the directions will be \textit{aligned}  or $\textit{anti-aligned}$ depending on the sign of $\cos \theta_1^{(1)} \cos \theta_1^{(2)}$. \todo{do we want to put some synthetic figure here showing these cases. like we could have something where its just $q_1 = e_1$, $q_2 = e_2$, and then show the different cases of what directions we stretch.}


==> checklist.tex <==



\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Sections \ref{sec: Stretching} and \ref{sec: Autoencoders}.}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{sec: Conclusion}} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section \ref{sec: Conclusion}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{All assumptions are stated in Sections \ref{sec: Stretching} and  \ref{sec: Autoencoders}} 
	\item Did you include complete proofs of all theoretical results?
    \answerYes{All proofs are provided in the Appendix.} 
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} \textcolor{red}{TODO link to code}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} 
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}. 
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We provide this in the Appendix.} 
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{All citations for datasets are present in \ref{sec: Applications}.}
  \item Did you mention the license of the assets?
    \answerYes{See citations discussed above.} 
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We provide a link to our code in \textcolor{red}{TODO}.} 
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{} 
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> sections/checklist.tex <==


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Sections \ref{sec: Stretching} and \ref{sec: Autoencoders}.}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{sec: Conclusion}} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section \ref{sec: Conclusion}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{All assumptions are stated in Sections \ref{sec: Stretching} and  \ref{sec: Autoencoders}} 
	\item Did you include complete proofs of all theoretical results?
    \answerYes{All proofs are provided in the Appendix.} 
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We provide a link to our code in the footnote at the end of the Abstract.} 
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} 
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}. 
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We provide this in the Appendix.} 
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{All citations for datasets are present in Section \ref{sec: Applications}.}
  \item Did you mention the license of the assets?
    \answerYes{See citations discussed above.} 
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We provide a link to our code in the footnote at the end of the Abstract.} 
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{} 
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> sections/stretching_section/2d_gaussian_ommitted_arithmetic.tex <==
Define the following helper variables:
$$a = \alpha + \beta, \quad b = \alpha - \beta, \quad  x = \sqrt{c^2 + 4} + c, \quad  y = \sqrt{c^2 + 4} - c, z = a^2 + b^2, r=\alpha^2 + \beta^2, s = \alpha^2 - \beta^2$$
Note the following:
\begin{align*}
    z &= 2(\alpha^2 + \beta^2)\\
    z^2 &= 4(\alpha^2 + \beta^2)^2\\
    x + y &= 2 \sqrt{c^2 + 4}\\
    xy &= 4\\
    x^2 + y^2 &= 4(c^2 + 2)\\
    ab &= \alpha^2 - \beta^2\\
    abz &= 2(\alpha^4 - \beta^4)\\
    a^2b^2 &= (\alpha^2 - \beta^2)^2
\end{align*}
    
Then we have that 
\begin{align*}
    E[B] &= \begin{bmatrix}
    a & b\\
    b & a
    \end{bmatrix}, q_{\Sigma_1} = \begin{bmatrix} 2 \\ x \end{bmatrix}, q_{\Sigma_2} = \begin{bmatrix} 2 \\ y \end{bmatrix}\\
    E[Bq_{\Sigma_1}] &= \begin{bmatrix} 2a + bx \\ 2b + ax \end{bmatrix} \quad E[Bq_{\Sigma_2}] = \begin{bmatrix} 2a + by \\ 2b + ay \end{bmatrix}\\
\end{align*}
We first take the dot product:
\begin{align*}
     E[Bq_{\Sigma_1}]^T E[Bq_{\Sigma_2}] &=  4a^2 + 2aby + 2abx + b^2xy + 4b^2 + 2bay + 2bax + a^2xy\\
     &= 8z + 4ab(x+y)\\
     &= 8(2(\alpha^2 + \beta^2) + (\alpha^2 - \beta^2) \sqrt{c^2 + 4})
\end{align*}
We then take the norms:
\begin{align*}
    ||E[Bq_{\Sigma_1}]||_2^2 &= (2a+bx)^2 + (2b + ax)^2\\
    &= 4a^2 + 4bax + b^2x^2 + 4b^2 + 4bax + a^2x^2\\
    &= 4(a^2 + b^2) + 8bax + x^2(a^2 + b^2)\\
    &= (x^2 + 4)z + 8abx\\
    ||E[Bq_{\Sigma_2}]||_2^2 &= (y^2 + 4)z + 8aby\\
     ||E[Bq_{\Sigma_1}]||_2^2 ||E[Bq_{\Sigma_2}]||_2^2 &= ((x^2 + 4)z + 8abx)((y^2 + 4)z + 8aby)\\
     &= (x^2+4)(y^2+4)z^2 + (x^2+4)z*8aby + (y^2+4)z * 8abx + 64a^2b^2xy\\
     &= (x^2+4)(y^2+4)z^2  + 8abz(y(x^2+4) + x(y^2+4)) + 256a^2b^2\\
     (x^2+4)(y^2+4)z^2 &= (x^2y^2 + 4x^2 + 4y^2 + 16)z^2\\
     &= (32 + 4(x^2 + y^2))(z^2)\\
     &= (32 + 16(c^2+2))(z^2)\\
     &= 4(64 + 16c^2)(\alpha^2 + \beta^2)^2\\
     &= 64(4 + c^2)(\alpha^2 + \beta^2)^2\\
     8abz(y(x^2+4) + x(y^2+4)) &= 8abz(x^2y + 4y + xy^2 + 4x)\\
     &= 8abz(4x + 4y + 4y + 4x)\\
     &= 64abz(x+y)\\
     &= 256(\alpha^4 - \beta^4)(\sqrt{c^2 + 4})\\
     256a^2b^2 &= 256(\alpha^2 - \beta^2)^2\\
     ||E[Bq_{\Sigma_1}]||_2^2 ||E[Bq_{\Sigma_2}]||_2^2 &= 64(4 + c^2)(\alpha^2 + \beta^2)^2 + 256(\alpha^4 - \beta^4)(\sqrt{c^2 + 4}) + 256(\alpha^2 - \beta^2)^2\\
     &= 64\left((4 + c^2)(\alpha^2 + \beta^2)^2 + 4(\alpha^4 - \beta^4)(\sqrt{c^2 + 4}) + 4(\alpha^2 - \beta^2)^2 \right)\\
     &= 64\left( (c^2+4)r^2 + 4rs\sqrt{c^2+4} + 4s^2 \right)\\
     &= 64(\sqrt{c^2 + 4}r + 2s)^2\\
     &= 64\left(\sqrt{c^2+4}(\alpha^2 + \beta^2) + 2(\alpha^2 - \beta^2)\right)^2\\
\end{align*}

Then combining the two we have:
\begin{align*}
    \frac{E[Bq_{\Sigma_1}]^T E[Bq_{\Sigma_2}]}{\sqrt{||E[Bq_{\Sigma_1}]||_2^2 ||E[Bq_{\Sigma_2}]||_2^2}} &= \frac{2(\alpha^2 + \beta^2) + (\alpha^2 - \beta^2) \sqrt{c^2 + 4}}{(\alpha^2 + \beta^2)\sqrt{c^2+4} + 2(\alpha^2 - \beta^2)}\\
    &=  \frac{2 + \gamma \sqrt{c^2 + 4}}{2\gamma + \sqrt{c^2 + 4}} , \quad \gamma = \frac{(\alpha^2 - \beta^2)}{(\alpha^2 + \beta^2)}
\end{align*}


==> sections/stretching_section/2d_gaussian_stretch_previous_draft.tex <==
\begin{lemma}
Consider the setting in Lemma \ref{lemma: XXT}, where $X_1, X_2 \in \mathbb{R}^{2 \times n}$. Let $X_1 \sim \mathcal{N}(e_1, \Sigma_1), X_2 \sim \mathcal{N}(e_2, \Sigma_2)$. Let $v = [1,1]^T$, $\hat{v} = \frac{[1,1]^T}{\sqrt{2}}$, and
$$D_1 = \begin{bmatrix} c & 0 \\ 0 & 1 \end{bmatrix}, \Sigma_1 = D_1 + vv^T = D_1 + J$$
$$D_2 = \begin{bmatrix} 1 & 0 \\ 0 & c \end{bmatrix}, \Sigma_2 = D_2 + vv^T = D_2 + J$$

Then before autoencoding, the cosine distance between the first principal directions of $X_1$ and $X_2$ is
$$ \cos(\theta_c) = \frac{2}{\sqrt{4 + (c-1)^2}}$$
and the cosine distance between the principal directions of the linearly autoencoded $X_1, X_2$, having set $A^{(0)} = 0, B^{(0)} = \left(\frac{1}{n}XX^T\right)^k$, is
$$\cos(\theta_c') = \frac{\alpha^2(c+5) - \beta^2(c+1)}{\sqrt{(\alpha^2(c+5) - \beta^2(c+1))^2 + 4 \alpha^2 \beta^2 (c-1)^2}}$$
for
$$\alpha = (\Sigma_B)_1 = \sqrt{\frac{(c+6)^{2k}}{2} + \sqrt{1 + \frac{(c+6)^{4k}}{4}}}, \beta = (\Sigma_B)_2 = \sqrt{\frac{(2+c)^{2}}{2} + \sqrt{1 + \frac{(2+c)^{4}}{4}}}$$

Moreover, 
$$cos(\theta_c) < cos(\theta_c'), \quad \forall c> 1$$ 
\textcolor{blue}{Saachi: This last statement is just from the plot for now}

\end{lemma}

Let $\lambda_i$ be the $i$th eigenvalue of $XX^T$. By Theorem \ref{theorem: two layer linear autoencoder}, if we initialize $A^{(0)}=0$ and  $B^{(0)} = \frac{1}{n} (XX^T)^k = U_X \Sigma_B U_X^T$, then after gradient descent we have:
$$B = U_X \Sigma_B U_X^T, (\Sigma_B)_i = \sqrt{\frac{\lambda_i^{2}}{2} + \sqrt{1 + \frac{\lambda_i^{4}}{4}}}$$

For our particular setting, from Theorem \ref{lemma: XXT},  we can calculate the expected value of $B^{(0)}$
$$E[B^{(0)}] = \mathbb{E}_{X_1, X_2}[\frac{1}{n} XX^T] = (2+c) I + 2 J = (2+c) I + 4\hat{v}\hat{v}^T$$
with eigenvectors $\hat{v}$ and $\hat{u} = [1, -1]^T/\sqrt{2}$ with eigenvalues:
$\lambda_1 = (c + 6), \lambda_2 = (2+c)$.

Then we have 

\noindent\fbox{%
    \parbox{\textwidth}{%
$$\alpha = (\Sigma_B)_1 = \sqrt{\frac{(c+6)^{2k}}{2} + \sqrt{1 + \frac{(c+6)^{4k}}{4}}}, \beta = (\Sigma_B)_2 = \sqrt{\frac{(2+c)^{2}}{2} + \sqrt{1 + \frac{(2+c)^{4}}{4}}}$$
and eigenvectors $\hat{v}$ and $\hat{u}$.
    }%
}
Then let $U_X$ be:
$$U_X = \begin{bmatrix} \hat{v} & \hat{u} \end{bmatrix} = \frac{1}{\sqrt{2}}\begin{bmatrix}1 & 1 \\ 1 & -1\end{bmatrix}$$

Then we have:
\begin{align*}B &= \frac{1}{2}
\begin{bmatrix}1 & 1 \\ 1 & -1\end{bmatrix}
\begin{bmatrix} \alpha & 0 \\ 0 & \beta \end{bmatrix}
\begin{bmatrix}1 & 1 \\ 1 & -1\end{bmatrix}\\
&= \frac{1}{2}
\begin{bmatrix}\alpha & \beta \\ \alpha & -\beta\end{bmatrix}
\begin{bmatrix}1 & 1 \\ 1 & -1\end{bmatrix}\\
&=  \frac{1}{2} \begin{bmatrix} \alpha + \beta & \alpha - \beta \\ \alpha - \beta & \alpha + \beta\end{bmatrix}\\
&= \frac{1}{2}(\alpha J + \beta \tilde{J})
\end{align*}
Where 
$$\tilde{J} = \begin{bmatrix} 1 & -1 \\ -1 & 1 \end{bmatrix}$$

First note that:
$$JJ = 2J, \quad \tilde{J} J = 0, \quad  JD_iJ = (c+1)J, \quad \tilde{J}D_i\tilde{J} = (c+1) \tilde{J}$$
$$\tilde{J}D_1J + JD_1\tilde{J} = (2c-2)\text{diag}([1, -1])$$
$$\tilde{J}D_2J + JD_2\tilde{J} = (2c-2)\text{diag}([-1, 1])$$


Then what is the expected covariance of the centered $X_i$ after autoencoding?:
\begin{align*}
Cov(BX_i) = E&[(BX_i - E[BX_i])(BX_i - E[BX_i])^T]\\
&= B\Sigma_1B^T\\
&= \frac{1}{4} (\alpha J + \beta \tilde{J}) (D_i + J) (\alpha J + \beta \tilde{J})\\
&= \frac{1}{4} (\alpha J D_i + \beta \tilde{J} D_i + \alpha J J + \beta \tilde{J} J) (\alpha J + \beta \tilde{J})\\
&= \frac{1}{4} (\alpha J D_i + \beta \tilde{J} D_i + 2 \alpha J) (\alpha J + \beta \tilde{J})\\
&= \frac{1}{4} (\alpha^2 J D_i J + \beta \alpha \tilde{J} D_i J + 2 \alpha^2 J J + \alpha \beta J D_i \tilde{J} + \beta ^2\tilde{J} D_i \tilde{J} + 2 \alpha \beta J  \tilde{J})\\
&= \frac{1}{4}(\alpha^2 (c+1) J + \alpha \beta(\tilde{J} D_i J + J D_i \tilde{J}) + 4 \alpha^2 J + \beta^2 (c+1) \tilde{J})\\
\end{align*}
For $X_1$ this is:
\begin{align*}
Cov(BX_1)   &= \frac{1}{4} (\alpha^2 (c+5)J + \alpha \beta (2c-2)\text{diag}([1, -1])  + \beta^2(c+1) \tilde{J})\\
&= \frac{1}{4} \begin{bmatrix} 
\alpha^2(c+5) + 2\alpha \beta(c-1) + \beta^2(c+1) & \alpha^2(c+5) - \beta^2(c+1)\\
 \alpha^2(c+5) - \beta^2(c+1) & \alpha^2(c+5) - 2\alpha \beta(c-1) + \beta^2(c+1)
\end{bmatrix}
\end{align*}
And for $X_2$ we simply flip to get:
\begin{align*}
Cov(BX_2) &= \frac{1}{4} \begin{bmatrix} 
\alpha^2(c+5)  - 2\alpha \beta(c-1) + \beta^2(c+1) & \alpha^2(c+5) - \beta^2(c+1)\\
 \alpha^2(c+5) - \beta^2(c+1) & \alpha^2(c+5) + 2\alpha \beta(c-1) + \beta^2(c+1)
\end{bmatrix}
\end{align*}

% use formula from here to get eigenvectors and values http://scipp.ucsc.edu/~haber/ph116A/diag2x2_11.pdf

Let $r = \alpha^2(c+5)$, $s = 2\alpha \beta(c-1)$, $t = \beta^2(c+1)$. Then the above matrices have the form:
$$
Cov(BX_1) = \begin{bmatrix}
r + s + t & r-t\\
r-t & r- s + t
\end{bmatrix}
$$
$$
Cov(BX_2) = \begin{bmatrix}
r - s + t & r-t\\
r-t & r + s + t
\end{bmatrix}
$$

$Cov(BX_1)$ has eigenvalues:
\begin{align*}
    \lambda(Cov(BX_1)) = r + t \pm \sqrt{s^2 + (r-t)^2}
\end{align*}
and eigenvectors:
\begin{align*}
    (q_{(BX_1)})_1 = \begin{bmatrix} r - t \\ \sqrt{s^2 + (r-t)^2} + s\end{bmatrix}, \quad
    (q_{(BX_1)})_2 = \begin{bmatrix} r - t \\ -\sqrt{s^2 + (r-t)^2} + s\end{bmatrix}
\end{align*}

and similarly $Cov(BX_2)$ has eigenvalues:
\begin{align*}
    \lambda(Cov(BX_1)) = r + t \pm \sqrt{s^2 + (r-t)^2}
\end{align*}
and eigenvectors:
\begin{align*}
    (q_{(BX_1)})_1 = \begin{bmatrix} r - t \\ \sqrt{s^2 + (r-t)^2} - s\end{bmatrix}, \quad
    (q_{(BX_1)})_2 = \begin{bmatrix} r - t \\ -\sqrt{s^2 + (r-t)^2} - s\end{bmatrix}
\end{align*}

We want the cosine distance between $(q_{(BX_1)})_1$ and $(q_{(BX_1)})_1$ is:
\begin{align*}
    (q_{(BX_1)})_1 \cdot (q_{(BX_1)})_2  &= (r-t)^2 + s^2 + (r-t)^2 - s^2\\
    &= 2 (r-t)^2\\
    ||(q_{(BX_1)})_1||_2^2 &= (r-t)^2 + s^2 + s^2 + (r-t)^2 +2s \sqrt{s^2 + (r-t)^2}\\
    &= 2(r-t)^2 + 2s^2 + 2s \sqrt{s^2 + (r-t)^2}\\
    ||(q_{(BX_1)})_2||_2^2 &= (r-t)^2 + s^2 + s^2 + (r-t)^2  - 2s \sqrt{s^2 + (r-t)^2}\\
    &= 2(r-t)^2 + 2s^2 - 2s \sqrt{s^2 + (r-t)^2}\\
    ||(q_{(BX_1)})_1||_2^2 ||(q_{(BX_1)})_2||_2^2 &= 4 (((r - t)^2 + s^2)^2 - s^2 (s^2 + (r-t)^2))\\
    &= 4((r-t)^2 + s^2)(r-t)^2\\
    \cos(\theta') &= \frac{(r-t)}{\sqrt{((r-t)^2 + s^2)}}\\
    &= \frac{\alpha^2(c+5) - \beta^2(c+1)}{\sqrt{(\alpha^2(c+5) - \beta^2(c+1))^2 + 4 \alpha^2 \beta^2 (c-1)^2}}
\end{align*}
The original eigenvalues of $\Sigma_1 = \begin{bmatrix} c+1 & 1 \\ 1 & 2 \end{bmatrix}$ and $\Sigma_2 =  \begin{bmatrix} 2 & 1 \\ 1 & c+1 \end{bmatrix}$ 
\begin{align*}
    \lambda &= \frac{1}{2} (c+3 \pm \sqrt{(c-1)^2 + 4}\\
\end{align*}
With eigenvectors:
$$(q_{(\Sigma_1})_1 = \begin{bmatrix} 2 \\ 1 - c + \sqrt{(c-1)^2 + 4}  \end{bmatrix},
(q_{(\Sigma_1})_2 = \begin{bmatrix} 2 \\ 1 - c - \sqrt{(c-1)^2 + 4}  \end{bmatrix}$$
$$(q_{(\Sigma_2})_1 = \begin{bmatrix} 2 \\ c-1 + \sqrt{(c-1)^2 + 4}  \end{bmatrix},
(q_{(\Sigma_2})_2 = \begin{bmatrix} 2 \\ c-1 - \sqrt{(c-1)^2 + 4}  \end{bmatrix}$$

We again find the cosine distance:
\begin{align*}
    (q_{(\Sigma_1})_1 \cdot (q_{(\Sigma_1})_2 &= 4 + (c-1)^2 + 4 - (c-1)^2\\
    &= 8\\
    || (q_{(\Sigma_1})_1 ||_2^2 &= 4 + (c-1)^2 + (c-1)^2 + 4 - 2 (c-1) \sqrt{(c-1)^2 + 4}\\
    &= 8 + 2(c-1)^2 - 2 (c-1) \sqrt{(c-1)^2 + 4}\\
    || (q_{(\Sigma_1})_2 ||_2^2 &= 4 + (c-1)^2 + (c-1)^2 + 4 + 2 (c-1) \sqrt{(c-1)^2 + 4}\\
    &= 8 + 2(c-1)^2 + 2 (c-1) \sqrt{(c-1)^2 + 4}\\
    || (q_{(\Sigma_1})_1 ||_2^2 || (q_{(\Sigma_1})_2 ||_2^2 &= 4(4 + (c-1)^2)^2 - 4(c-1)^2 ((c-1)^2 + 4)\\
    &= 4(4 + (c-1)^2)(4)\\
    \cos(\theta) &= \frac{2}{\sqrt{4 + (c-1)^2}}
\end{align*}
Thus our before and after cosine distances of the major principal directions are 

\noindent\fbox{%
    \parbox{\textwidth}{%
    $$ \cos(\theta) = \frac{2}{\sqrt{4 + (c-1)^2}}, \quad \cos(\theta') = \frac{\alpha^2(c+5) - \beta^2(c+1)}{\sqrt{(\alpha^2(c+5) - \beta^2(c+1))^2 + 4 \alpha^2 \beta^2 (c-1)^2}}$$
    for
    $$\alpha = (\Sigma_B)_1 = \sqrt{\frac{(c+6)^{2k}}{2} + \sqrt{1 + \frac{(c+6)^{4k}}{4}}}, \beta = (\Sigma_B)_2 = \sqrt{\frac{(2+c)^{2}}{2} + \sqrt{1 + \frac{(2+c)^{4}}{4}}}$$
    }%
}

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{Figures/translation_alignment_plot_cosine_sims.png}
    \caption{We plot the cosine distance (original and autoencoded for different polynomial $k$) between the top principal direction of the two gaussians for increasing values of $c$.
}
    \label{fig:Gaussian 2D alignment}
\end{figure}

